LEGOStore: A Linearizable Geo-Distributed Store Combining Replication and Erasure Coding

We design and implement LEGOStore, an erasure coding (EC) based linearizable data store over geo-distributed public cloud data centers (DCs). For such a data store, the confluence of the following factors opens up opportunities for EC to be latency-competitive with replication: (a) the necessity of communicating with remote DCs to tolerate entire DC failures and implement linearizability; and (b) the emergence of DCs near most large population centers. LEGOStore employs an optimization framework that, for a given object, carefully chooses among replication and EC, as well as among various DC placements to minimize overall costs. To handle workload dynamism, LEGOStore employs a novel agile reconfiguration protocol. Our evaluation using a LEGOStore prototype spanning 9 Google Cloud Platform DCs demonstrates the efficacy of our ideas. We observe cost savings ranging from moderate (5-20\%) to significant (60\%) over baselines representing the state of the art while meeting tail latency SLOs. Our reconfiguration protocol is able to transition key placements in 3 to 4 inter-DC RTTs ($<$ 1s in our experiments), allowing for agile adaptation to dynamic conditions.

==> 6implementation.tex <==
% \vspace{-5pt}
\section{Salient Implementation Aspects}
\label{sec:impl}

%\bu{

%Need to address: what is the meta data overhead per key? Clarify why LEGOStore doesn't need another key-value store  as an SOSP reviewer had thought.  
%}

We implement our  optimizer %(our heuristic approach) 
using Python3.
% in about 1K LOC;  baselines add another 1K LOC.
Since finding the configurations can be done in parallel with each other, we execute up to 48 instances of the optimizer in parallel spanning 8 \emph{e2-standard-4} GCP VMs.\footnote{Our optimizer takes \bu{XXX} msec for each workload on average for $f$=1.}  We implement our LEGOStore prototype in C++11 using about 5.5K LOC. Our prototype uses the {\tt liberasurecode} library's~\cite{liberasurecode}  Reed-Solomon backend for encoding and decoding data in CAS. 
%Figure~\ref{fig:impl} depicts key software components comprising our LEGOStore prototype.
We refer to LEGOStore's users and clients \& servers of our protocols as its {\em data plane}; we call the per-DC metadata servers, the optimizer and reconfiguration controllers its {\em control plane}. \lego's source code is available under the Apache license 2.0 at \href{https://github.com/shahrooz1997/LEGOstore}{github.com/shahrooz1997/LEGOstore}.

\noindent {\bf Data Plane:} A user application (simply user) needs to link the \lego~library %(instead of the key-value store it was using) 
and ensure it uses \lego's API. The library implements logic for the user to interact with the appropriate (ABD or CAS) client. 
LEGOStore maintains a pool of {\em compute nodes} (VMs) (GCP `custom-1-1024' instance types) that run the client and server protocols and store keys using the RocksDB~\cite{rocksdb} database engine.

Each DC maintains a meta-data server (MDS) locally %in its storage layer 
that contains configurations for keys that the clients within it have served and that have not yet been deleted. {\em LEGOStore does not have to have a centralized MDS} with corresponding freedom from concerns related to the failure of such an MDS. When a client does not find a key in the local MDS, it issues queries to other DCs (e.g., in increasing order of RTTs) to learn the key's configuration.

\noindent {\bf Control Plane:}   LEGOStore's control plane comprises the two types of elements for each key described in Section~\ref{sec:interface}: (i) the optimizer and (ii) the reconfiguration controller. Neither of these components is tied to a particular DC location (e.g., See Section~\ref{sec:reconfig-whenwhat} for discussion regarding controller placement). 


==> LegoStore-VLDB22CameraReady-arxiv(3)/1introduction.tex <==
\section{Introduction}

%\bu{EC can save costs over replication. EC's potential has become  established as a cost saver {\em within a data center} enabled by xyz findings/insights/technical advances.}

Consistent geo-distributed key-value (KV) stores are crucial building blocks of %infrastructural component 
%large-scale 
modern Internet-scale services including databases and web applications. %Of the various consistency criteria, 
Strong consistency (i.e., linearizability) is especially %particularly 
preferred by users for the ease of development and testing it offers. % building applications. 
As a case in point, the  hugely popular S3 store from Amazon Web Services (AWS), in essence a KV store with a GET/PUT interface,  was recently re-designed to switch its consistency model from eventual to linearizable~\cite{s3-blog}. However, because of the inherent lower bound in  \cite{attiya1994sequential}, linearizable KV stores inevitably incur significant latency and cost overheads compared to weaker consistency models such as causal and eventual consistency. These drawbacks are particularly pronounced in the geo-distributed setting because of the  high inter-data center networking costs, and large network latencies (see Table~\ref{tab:net+rtt}). To further exacerbate the problem, dynamic phenomena such as shifts in arrival rates, appearance of clients in new locations far from where data is stored,  increase in network delays, etc., can lead to gaps between predicted and actual performance both in terms of costs and tail latencies. 

\begin{table*}[ht]\centering
\footnotesize
\caption{Storage and VM prices for the 9 GCP data centers that our prototype spans. We use custom VMs with 1 core and 1 GB of RAM from General-purpose machine type family to run the \lego's servers and Standard provisioned space for its storage~\cite{gcp-pricing}.}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lrccccccccc}\toprule
&\multicolumn{9}{c}{\cellcolor[HTML]{fff2cc}GCP data center location} \\\cmidrule{2-10}
&\cellcolor[HTML]{d9d9ff}Tokyo &\cellcolor[HTML]{d9d9ff}Sydney &\cellcolor[HTML]{d9d9ff}Singapore &\cellcolor[HTML]{d9d9ff}Frankfurt &\cellcolor[HTML]{d9d9ff}London &\cellcolor[HTML]{d9d9ff}Virginia &\cellcolor[HTML]{d9d9ff}São Paulo &\cellcolor[HTML]{d9d9ff}Los Angeles &\cellcolor[HTML]{d9d9ff}Oregon \\\cmidrule{2-10}
\cellcolor[HTML]{d9ead3}Storage (\$/GB.Month) &0.052 &0.054 &0.044 &0.048 &0.048 &0.044 &0.06 &0.048 &0.04 \\
\cellcolor[HTML]{d9ead3}Virtual machine (\$/hour) &0.0261 &0.0283 &0.0253 &0.0262 &0.0262 &0.0226 &0.0310 &0.0248 &0.0215 \\
\bottomrule
\end{tabular}}
\label{tab:dcs}
% \vspace{-15pt}
\end{table*}

\begin{table*}[ht]\centering
\footnotesize
\caption{Diverse RTTs and network pricing for 9 chosen GCP data centers. 
%Prices of the form (GCP data center=Tokyo, User location=Tokyo) are non-zero because the recipients are external to GCP. Network traffic between GCP DCs is priced differently but also shows geographic diversity; for such traffic the price for (Tokyo, Tokyo) would be 0.
The RTTs are measured between VMs placed within the DCs; they would be higher if one of the VMs were external to GCP but not by enough to change the outcome of our optimizer. For the same general recipient location, the outbound network prices are sometimes higher if the recipient is located outside of GCP (egress pricing) but these prices exhibit a similar geographical diversity ~\cite{gcp-network-pricing}.}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{llccccccccccccccccccc}\toprule
& &\multicolumn{18}{c}{\cellcolor[HTML]{fff2cc}User location} \\\cmidrule{3-20}
& &\multicolumn{2}{c}{\cellcolor[HTML]{d9d9ff}Tokyo} &\multicolumn{2}{c}{\cellcolor[HTML]{d9d9ff}Sydney} &\multicolumn{2}{c}{\cellcolor[HTML]{d9d9ff}Singapore} &\multicolumn{2}{c}{\cellcolor[HTML]{d9d9ff}Frankfurt} &\multicolumn{2}{c}{\cellcolor[HTML]{d9d9ff}London} &\multicolumn{2}{c}{\cellcolor[HTML]{d9d9ff}Virginia} &\multicolumn{2}{c}{\cellcolor[HTML]{d9d9ff}São Paulo} &\multicolumn{2}{c}{\cellcolor[HTML]{d9d9ff}Los Angeles} &\multicolumn{2}{c}{\cellcolor[HTML]{d9d9ff}Oregon} \\\cmidrule{3-20}
& &\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}n/w\\ price\\(\$/GB)\end{tabular} &\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}\rotatebox[origin=c]{90}{Latency (ms)}\end{tabular}
&\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}n/w\\ price\\(\$/GB)\end{tabular} &\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}\rotatebox[origin=c]{90}{Latency (ms)}\end{tabular}
&\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}n/w\\ price\\(\$/GB)\end{tabular} &\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}\rotatebox[origin=c]{90}{Latency (ms)}\end{tabular}
&\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}n/w\\ price\\(\$/GB)\end{tabular} &\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}\rotatebox[origin=c]{90}{Latency (ms)}\end{tabular}
&\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}n/w\\ price\\(\$/GB)\end{tabular} &\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}\rotatebox[origin=c]{90}{Latency (ms)}\end{tabular}
&\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}n/w\\ price\\(\$/GB)\end{tabular} &\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}\rotatebox[origin=c]{90}{Latency (ms)}\end{tabular}
&\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}n/w\\ price\\(\$/GB)\end{tabular} &\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}\rotatebox[origin=c]{90}{Latency (ms)}\end{tabular}
&\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}n/w\\ price\\(\$/GB)\end{tabular} &\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}\rotatebox[origin=c]{90}{Latency (ms)}\end{tabular}
&\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}n/w\\ price\\(\$/GB)\end{tabular} &\cellcolor[HTML]{b6d7a8}\begin{tabular}{@{}c@{}}\rotatebox[origin=c]{90}{Latency (ms)}\end{tabular}
 \\\midrule
\cellcolor[HTML]{fff2cc}&\cellcolor[HTML]{d9d9ff}Tokyo & - &2 &0.15 &115 &0.12 &70 &0.12 &226 &0.12 &218 &0.12 &148 &0.12 &253 &0.12 &100 &0.12 &90 \\
\cellcolor[HTML]{fff2cc}&\cellcolor[HTML]{d9d9ff}Sydney &\cellcolor[HTML]{efefef}0.15 &\cellcolor[HTML]{efefef}115 &\cellcolor[HTML]{efefef}- &\cellcolor[HTML]{efefef}2 &\cellcolor[HTML]{efefef}0.15 &\cellcolor[HTML]{efefef}94 &\cellcolor[HTML]{efefef}0.15 &\cellcolor[HTML]{efefef}289 &\cellcolor[HTML]{efefef}0.15 &\cellcolor[HTML]{efefef}277 &\cellcolor[HTML]{efefef}0.15 &\cellcolor[HTML]{efefef}204 &\cellcolor[HTML]{efefef}0.15 &\cellcolor[HTML]{efefef}291 &\cellcolor[HTML]{efefef}0.15 &\cellcolor[HTML]{efefef}139 &\cellcolor[HTML]{efefef}0.15 &\cellcolor[HTML]{efefef}162 \\
\cellcolor[HTML]{fff2cc}&\cellcolor[HTML]{d9d9ff}Singapore &0.09 &72 &0.15 &94 &- &2 &0.09 &202 &0.09 &203 &0.09 &214 &0.09 &319 &0.09 &165 &0.09 &166 \\
\cellcolor[HTML]{fff2cc}&\cellcolor[HTML]{d9d9ff}Frankfurt &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}229 &\cellcolor[HTML]{efefef}0.15 &\cellcolor[HTML]{efefef}289 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}201 &\cellcolor[HTML]{efefef}- &\cellcolor[HTML]{efefef}2 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}15 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}89 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}202 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}153 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}139 \\
\cellcolor[HTML]{fff2cc}&\cellcolor[HTML]{d9d9ff}London &0.08 &222 &0.15 &280 &0.08 &204 &0.08 &15 &- &2 &0.08 &79 &0.08 &192 &0.08 &141 &0.08 &131 \\
\cellcolor[HTML]{fff2cc}&\cellcolor[HTML]{d9d9ff}Virginia &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}146 &\cellcolor[HTML]{efefef}0.15 &\cellcolor[HTML]{efefef}204 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}214 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}90 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}79 &\cellcolor[HTML]{efefef}- &\cellcolor[HTML]{efefef}2 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}116 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}68 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}58 \\
\cellcolor[HTML]{fff2cc}&\cellcolor[HTML]{d9d9ff}São Paulo &0.08 &252 &0.15 &292 &0.08 &317 &0.08 &202 &0.08 &192 &0.08 &117 &- &1 &0.08 &155 &0.08 &172 \\
\cellcolor[HTML]{fff2cc}&\cellcolor[HTML]{d9d9ff}Los Angeles &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}101 &\cellcolor[HTML]{efefef}0.15 &\cellcolor[HTML]{efefef}139 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}180 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}153 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}142 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}67 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}155 &\cellcolor[HTML]{efefef}- &\cellcolor[HTML]{efefef}2 &\cellcolor[HTML]{efefef}0.08 &\cellcolor[HTML]{efefef}26 \\
\multirow{-9}{*}{\cellcolor[HTML]{fff2cc}\rotatebox[origin=c]{90}{GCP data center}}&\cellcolor[HTML]{d9d9ff}Oregon &0.08 &95 &0.15 &164 &0.08 &165 &0.08 &142 &0.08 &131 &0.08 &58 &0.08 &173 &0.08 &26 &- &2 \\
\bottomrule
\end{tabular}}
\label{tab:net+rtt}
% \vspace{-20pt}
\end{table*}

We design LEGOStore, a geo-distributed linearizable KV store (with the familiar GET/PUT or read/write API), meant for a global user-base. LEGOStore procures its resources from a cloud provider's fleet of data centers (DCs) like many  storage service providers~\cite{evernote,overleaf,aws-outage-github}. Since an entire DC may become unavailable~\cite{aws-outage-github,azure-outage1,azure-outage2,Veeraraghavan:2018:MMD:3291168.3291196}, LEGOStore employs  redundancy across geo-distributed DCs to operate despite such events. LEGOStore's goal is to {\em  offer  tail  latency  service-level objectives (SLOs) that are predictable and robust in the face of myriad sources of dynamism at a low cost}. For achieving these properties, LEGOStore is built upon the following three pillars:

%\noindent 
\textbf{1. Erasure Coding (EC)} is a generalization of replication that is more storage-efficient than replication for a given fault tolerance. A long line of research  %The storage savings enabled by EC in the face of rapidly growing data volumes and  the emergence of highly optimized EC libraries %optimized to specific hardware 
%that reduce encoding/decoding overheads~\cite{burihabwa2016performance,intel-isal,rashmi2016ec} have %particularly 
has helped establish EC's efficacy {\em within a DC} or for weaker consistency needs. %; see Section~\ref{sec:related}. 
However, EC's efficacy in %the context of 
the linearizable geo-distributed setting is relatively %more recent and 
less well-understood.  Two recent works Giza~\cite{giza} and Pando~\cite{pando} demonstrate some aspects of EC's promise in the geo-\-distributed context. In particular, because EC allows fragmenting the data and storing it in a fault-tolerant manner, it leads to smaller storage costs and (more importantly) smaller inter-DC networking costs. However, the smaller-sized fragments inevitably require contacting more DCs and,  therefore, are thought to imply higher latencies in a first-order estimation. By comprehensively exploring a wide gamut of workload features and SLOs,  and careful design of the data placement and EC parameters through an optimization framework,  LEGOStore brings out the full potential of EC in the geo-distributed setting. 


%\noindent 
\textbf{2. %Fault-Tolerant Non-Blocking Protocols:
} 
LEGOStore adapts {\bf non blocking, leaderless, quorum based linearizability protocols} for both EC~\cite{cadambe2017coded} and replication~\cite{ABD_conference,ABD}. When used with carefully optimized quorums, these protocols help realize LEGOStore's goal of predictable performance (i.e.,  meeting latency SLOs with a very high likelihood as long as workload features match their predicted values considered by our optimization). A second important reason is that, when used in conjunction with a well-designed resource autoscaling strategy, the  latency resulting from non-blocking protocols depends primarily on its inter-DC latency and data transfer time components. %for using non-blocking protocols is that, with sufficient resource provisioning, they help eliminate performance degrading effects that high degrees of concurrency may have on user latencies if alternative consensus-based protocols were used.  Specifically, 
 This is in contrast with the  leader-based consensus used in Giza and Pando (see Figure~\ref{fig:concurrency} ). % that lead to poor performance for write-intensive workloads. 
While these works %consensus-based approaches 
may be able to offer lower latencies for certain workloads, they are susceptible to severe performance degradation under concurrency-induced contention. %Finally, our optimizer is carefully designed to pick from our 2 protocols and associated operational parameters to allow meeting SLOs at minimum cost. 


%\noindent 
\textbf{3. %Agile Reconfiguration:
} To offer robust SLOs in the face of dynamism, LEGOStore implements an {\bf agile reconfiguration mechanism}. LEGOStore continually weighs the pros and cons of changing the {\em configuration}\footnote{By the configuration of a key, we mean the following  aspects of its placement: (i) whether EC or replication is being used ; (ii) the EC parameters or replication degree being used; and (iii) the DCs that comprise various quorums. %; (iv) the optimized set of quorums to do operations from each client. Commenting out (iv) because optimized ideas haven't been introduced yet. 
} of a key or a group of keys via a cost-benefit analysis rooted in its cost/performance modeling.  %that underlies its optimization. 
If prompted by this  analysis, it uses a novel reconfiguration protocol to safely switch the configurations of concerned keys   without breaking linearizability. We have designed this reconfiguration protocol carefully and specifically to work alongside our GET/PUT protocols to keep its execution time small which,  in turn, allows us to limit the performance degradation experienced by user requests issued during a reconfiguration. 

\noindent 
{\bf Contributions:} %Our main contribution is the 
We design \lego, a cost-effective KV store with predictable tail latency  that adapts to dynamism. We develop an optimization framework that, for a group of keys with similar suitable workload features,  takes as input these features, and public cloud characteristics and determines configurations that satisfy SLOs at minimal cost. The configuration choice involves selecting one from a  family of linearizability protocols, and the protocol parameters that can include the degree of redundancy, DC placement, quorum sizes, and EC parameters. In this manner it selectively uses EC for its better storage/networking costs when allowed by latency goals, and uses replication otherwise. A key’s storage method may change over time based on changes in workload features. % (across replication and EC as well as in terms of parameters within each). %However, at any given time, a key’s storage method is fixed (either replication-based or EC-based). }  
We develop a %provably 
safe reconfiguration protocol, and an accompanying  heuristic cost/benefit analysis that allows \lego~ to control costs by dynamically adapting configurations. % in response to changes in workload features.

We build a prototype LEGOStore system.  We carry out extensive evaluations using our optimizer and prototype spanning 9 Google Cloud Platform (GCP) DCs. We get insights from our evaluation to make suitable modeling and protocol design choices. Because of our design, our prototype has close match with the performance predicted by the optimizer. Potential cost savings over baselines based on state-of-the-art works such as SPANStore~\cite{spanstore} and  Pando~\cite{pando} range from moderate (5-20\%) to significant (up to 60\%). The most significant cost savings emerge from carefully avoiding the use of DCs with high outbound network prices. Our work offers a number of general trends and insights relating workload and infrastructure properties to cost-effective realization of linearizability. Some of our findings are perhaps non-intuitive: (i) smaller EC-fragments do not always lead to lower costs (Section~\ref{subsubsec:opt-k-dep}); (ii) there exists a significant asymmetry between GETs and PUTs in terms of costs, and read-heavy workloads lead to different choices than write-heavy workloads (Section~\ref{subsec:asymmetry}); (iii) we find scenarios where the optimizer is able to exploit the lower costs of EC without a latency penalty (Section~\ref{subsec:ECvsrep}); and (iv) even when a majority of the requests to a key arise at a particular location, the DC near that location may not necessarily be used for this key in our optimizer's solution. 
    

==> LegoStore-VLDB22CameraReady-arxiv(3)/2background.tex <==
\section{Background}
\label{sec:back}

%LEGOStore's goal is to design a cost effective linearizable key value store over the public cloud that meets the service level latency objectives (SLOs) of the clients. 
\noindent {\bf Public Cloud Latencies and Pricing:} The lower bound of~\cite{attiya1994sequential,Attiya_Welch} implies that {\em both} GET and PUT operations in LEGOStore necessarily involve inter-DC latencies and data transfers %send values across nodes (DCs here), 
unlike with weaker consistency models. %As a consequence, latency of operations is lower bounded by inter-DC traversal time, and every operation also incurs  inter-DC messaging costs. 
%Public clouds having DCs at different locations across the globe implies that 
The latencies between users and various DCs of a public cloud provider span a large range. In Table~\ref{tab:net+rtt} we depict our measurements  of round-trip times (RTTs) between pairs of DCs out of a set of 9 Google Cloud Platform (GCP) data centers we use. The smallest RTTs are 15-20 msec while the largest exceed 300 msec; RTTs between nodes within the same DC are 1-2 msec and pale in comparison. Similarly, the prices for storage, computational, and network resources across DCs also exhibit geographical diversity as shown in Tables~\ref{tab:dcs} and~\ref{tab:net+rtt}. This diversity is the most prominent for data transfers---the cheapest per-byte transfer is  \$0.08/GB (e.g., London to Tokyo), the costliest is \$0.15/GB (e.g., Sydney to Tokyo). LEGOStore's design must carefully navigate these sources of diversity to meet latency SLOs at minimum cost. 



\noindent {\bf Our Choice of Consistent Storage Algorithms:} %{We are interested in designing a strongly consistent data store that is tolerant of DC failures.  Because of the lower bounds in ~\cite{attiya1994sequential,Attiya_Welch}, it is necessary for any protocol that satisfies our design requirements to incur at least one round trip to a quorum over the wide area network (WAN) during both read and write operations. 
Due to the lower bound mentioned above, in leader-based protocols (e.g., Raft~\cite{raft}), for the geo-distributed scenario of interest to us, one round trip time to the leader is inevitable. Using such leader-based protocols can drive up latency when the workload is distributed over a wide geographical area, and there is no leader node that is sufficiently close to all DCs so as to satisfy the SLO requirements. Such a design can also place excessive load on DCs that are more centrally located. %\bu{For Viveck: Should we say something about the complexity of handling leader failures?} 
Therefore, as such, we choose algorithms with leaderless, quorum-based protocols in our design and implementation. We describe these protocols (ABD for replication and CAS for EC) next. %For replicated keys, LEGOStore uses an algorithm, which we call \emph{ABD}\footnote{The name ``ABD'' comes from the authors, Attya, Bar-Noy and Dolev ~\cite{ABD_conference}.}  ~\cite{ABD_conference,ABD},  a \emph{quorum}-based leaderless protocol that offers non-blocking, linearizable GET and PUT operations \cite{herlihy90,lamport1979make}. This protocol is reviewed next.

%Next, we provide an overview of erasure coding and the linearizability  algorithms\footnote{In our protocol descriptions, we assume that all the GET/PUT operations are issued at \emph{clients} and the data is stored at servers.} used by LEGOStore.  


\noindent{\bf The ABD Algorithm:}\footnote{The name ``ABD'' comes from the authors, Attya, Bar-Noy and Dolev ~\cite{ABD_conference,ABD}.} 
  % provide fault-tolerance \todo{data availability?} to the system.
Let $N$ denote the degree of replication (specifically, spanning $N$ separate DCs) being used for the key under discussion. In the ABD algorithm, for a given key, each of the nodes (i.e., DCs) stores a (tag, value) pair, where the tag is a (logical timestamp, client ID) pair. The node replaces this tuple when it receives a value with a higher tag from a client operation.
   %The ABD protocol is shown in Figure \ref{}, we only overview the key aspects here. 
The PUT operation consists of two phases. The first phase, which involves a logical-time query, requires responses from a quorum of $q_1$ nodes, and the second phase, which involves sending the  new (tag, value) pair requires acknowledgements from a quorum of $q_2$ nodes. The GET operation also consists of two phases. The first phase again involves logical-time queries from a quorum of $q_1$ nodes and determining the highest of these tags.  The second ``write-back'' phase %is %only invoked if a predicate is not satisfied, and 
sends the  (tag, value) pair chosen from the first-phase responses to a quorum of $q_2$ nodes. %The second phase, which is crucial in ensuring linearizability in presence of concurrent writes, completes on receiving acknowledgements from $q_2$ nodes. 
If $q_1+q_2 > N$, then ABD guarantees linearizability. If $q_1, q_2 \leq N-f,$ then operations terminate so long as the number of node failures is at most $f.$  Note that this is a stronger liveness guarantee as compared to Paxos; ABD circumvents FLP impossibility \cite{FLP} because it implements a data type (read/write memory) that is weaker than consensus \vc{(see also  \cite{ABD_Djisktra} and Theorems 17.5, 17.9 in \cite{Lynch1996})}.  This liveness property translates into excellent robustness of operation latency (see Section~\ref{sec:concurrency}). See formal description of ABD in Appendix~\ref{app:ABD} of ~\cite{legostore-arxiv}.

Whereas the above vanilla ABD requires two phases for all its GET operations, a slight enhancement allows some (potentially many) GET operations to complete in only one phase; we refer to such a scenario as an ``Optimized GET,'' see details in \cite{legostore-arxiv}.
%  A GET operation becomes an  Optimized GET  if all the servers return the same (tag, value) pair in the first phase. This scenario occurs if there is no concurrent operation, and some previous operation to the same key has propagated the version to the servers in the quorum that responds to the client. Furthermore, to increase the recurrence of Optimized GET, we enhance the vanilla ABD algorithm to do an asynchronous phase after each PUT operation to propagate (tag, value) pair to servers that do not constitute $q_2$. The Optimized GET mirrors consensus protocols such as Paxos, where operations can complete in one phase in optimistic circumstances. 

%Our paper also involves an optimization for CAS that enables some GET operations to complete in one phase. %Since our optimization focuses on worst-case latencies, our modeling makes a conservative estimate that no operation performs an Optimized GET. A minor extension of our work can allow nodes to gossip the versions in the background (after the operation is complete) to increase the fraction of Optimized GETs for ABD protocol at an increased communication cost (See, e.g., \cite{pando} that performs such an optimization).





% \begin{table*}[!htb]\scriptsize

% \small\centering
% 	{\renewcommand{\arraystretch}{1}
% \renewcommand{\tabcolsep}{0.2cm}
% {
% 	\begin{tabular}[c]{|>{\color{blue}} c || >{\color{blue}}c |>{\color{blue}} c | >{\color{blue}}c | >{\color{blue}}c | >{\color{blue}}c | >{\color{blue}}c |}
  
% %  \parbox[t][0.40in][t]{0.6in}{Algorithm}& \multicolumn{3}{|c||}{\parbox{1.6in}{Worst-case among all executions.}} & \multicolumn{3}{|c|}{\parbox{1.90in}{Worst case among executions with bounded number of ongoing write operations, message delays, and rate of client failures.}} &\multicolumn{1}{|c|} {\parbox{0.9in}{Storage cost when there is no ongoing write operation\footnotemark .}}\\  
%   \hline %\rule{0pt}{8ex}
%   & \parbox[t][0.13 in][t]{0.8in}{PUT Comm. Cost} & PUT Latency & \parbox[t][0.13 in][t]{0.8in}{GET Comm. cost\footnote{}} &  \parbox[t][0.13 in][t]{0.8in}{GET Latency} & \parbox[t][0.13 in][t]{0.8in}{Storage cost} & \parbox{0.7in}{Remarks} \\[0ex]
%   \hline \rule{0pt}{6ex}
%   \parbox[t][0.25in][t]{0.2in}{CAS}& \parbox{0.4in}{$\frac{NB}{k}$} & $3$ Rounds & \parbox{0.4in}{$\frac{(N-K) B}{2K}$} & \parbox{0.4in}{2 rounds} & $\delta\frac{B}{k}$ & \parbox{1.7 in}{With efficient garbage collection, $\delta$ can be kept small; it is equal to $1$ for keys with sufficiently low arrival rates.}\\\hline \rule{0pt}{2ex}
% \parbox[t][0.42in][t]{0.2in}{ABD}& \parbox{0.4in}{$NB$} & \parbox{0.4in}{2 rounds}& \parbox{0.6in}{$(N-1) B$} & \parbox{0.4in}{$2$ rounds} &  $1$ & \parbox[t]{1.7 in}{ABD has an higher communication cost compared to CAS for GETs, even if $k=1$, since it propagates values in the write-back phase, whereas CAS only propagates metadata.} \\  \hline
% \end{tabular}}}
% % \vspace{0.1in}
% \caption{\color{blue}{Coarse cost comparison of replication (ABD) versus erasure coding (CAS). Costs reported are per GET/PUT operation, and the per-server storage cost. We assume that each value has $B$ bits and the metadata size is negligible. All quorum sizes are assumed to be $(N+k)/2$ for CAS and $(N+1)/2$ for ABD;   $N,k$ are assumed to be odd to ignore integer rounding. Latency is reported as the number of round trips of the protocol. }}
% \label{table:comparison}
% % \vspace{-0.3 in}
% \end{table*}
% \footnotetext{If an optimized GET is performed for ABD or CAS, the GET latency can be reduced to $1$ round. For ABD, the communication cost also reduces to $\frac{N-1}{2}$. }


\begin{table}[t]\centering
\footnotesize
\caption{Coarse cost comparison of replication (ABD) versus erasure coding (CAS). Costs reported are per GET/PUT operation, and the per-server storage cost. We assume that each value has $B$ bits and the metadata size is negligible. All quorum sizes are assumed to be $(N+k)/2$ for CAS and $(N+1)/2$ for ABD;   $N,k$ are assumed to be odd to ignore integer rounding. Latency is reported as the number of round trips of the protocol.}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{lcccccc}\toprule
&\cellcolor[HTML]{d9d9ff}PUT cost &\cellcolor[HTML]{d9d9ff}PUT latency &\cellcolor[HTML]{d9d9ff}GET cost &\cellcolor[HTML]{d9d9ff}GET latency &\cellcolor[HTML]{d9d9ff}Storage cost \\\cmidrule{2-6}
\cellcolor[HTML]{d9ead3}CAS\footnote{With efficient garbage collection, $\delta$ can be kept small; it is equal to $1$ for keys with sufficiently low arrival rates.} &$\frac{NB}{k}$ & $3$ rounds & $\frac{(N-K) B}{2K}$ & 2 rounds & $\delta\frac{B}{k}$ \\
\cellcolor[HTML]{d9ead3}ABD\footnote{ABD has a higher communication cost vs. CAS for GETs, even if $k=1$, since it propagates values in the write-back phase, whereas CAS only propagates metadata.} &$NB$ & 2 rounds& $(N-1) B$ & $2$ rounds & $1$ \\
\bottomrule
\end{tabular}
\label{table:comparison}
% \vspace{-15pt}
\end{center}
% \bigskip
\end{minipage}
\end{table}

\noindent \textbf{Erasure Coding:} Erasure coding (EC) is a generalization of replication that is attractive for modern storage systems because of its potential cost savings over replication. An $(N,K)$ Reed Solomon Code stores a value over $N$ nodes, with each node storing a codeword symbol %\todo{?} of 
of size $1/K$ of the original value, unlike replication where each node stores the entire value.  The value can be decoded from \emph{any} $K$ of the $N$ nodes, so the code tolerates  up to $f=N-K$ failures. On the other hand, replication duplicates the data $N=f+1$ times to tolerate $f$ failures. For a fixed value of $N$, EC leads to a $K$-fold reduction in storage cost compared to $N$-way replication for the same fault-tolerance. It also leads to a $K$-fold reduction in communication cost for PUTs, which  can be significant because of the inter-DC network transfer pricing. While this suggests that costs reduce with increasing $K$, we will see that the actual dependence of costs on $K$ in LEGOStore is far more complex (see Section~\ref{subsubsec:opt-k-dep}).

In EC-based protocols, GET operations require $K > 1$ nodes to respond with codeword symbols for %corresponding to 
the \emph{same} version of the key. However, due to asynchrony, different nodes may store different versions at a given time. Reconciling the different versions incurs additional communication overheads for EC-based algorithms. % as compared with ABD. \\ %
   
   
%The use of EC leads to structural changes in non-blocking linearizable protocols~\cite{CadambeCoded_NCA, cadambe2017coded, Dutta, Hendricks, GWGR}. 
 %in terms of communication. 
\noindent \textbf{The CAS Algorithm:}
We use the  \emph{coded atomic storage} (CAS) algorithm\footnote{{The algorithm in Appendix \ref{app:cas} of~\cite{legostore-arxiv} is a modification the algorithm in~\cite{CadambeCoded_NCA, cadambe2017coded} to allow for flexible quorum sizes, which in turn this exposes more cost-saving opportunities.} %\bu{CANDIDATE FOR REMOVAL?} Our ultimate scientific goal in this paper is to develop general insights for linearizable key-value stores that can use erasure coding, and several of our insights can be adapted/translated to other algorithms as well.
} of~\cite{CadambeCoded_NCA, cadambe2017coded}, described %formally 
in Appendix \ref{app:cas} of~\cite{legostore-arxiv}.   
In CAS, servers store a list of triples, each consisting of a tag, a codeword symbol, and a label that can be `pre' or `fin'.  The GET protocol operates in two phases like ABD; however, PUT operates in {\em three} phases. Similar to ABD, the first phase of PUT  acquires the latest tag. The second phase sends an encoded value to servers, and servers store this symbol with a `pre' label. The third phase propagates the `fin' label to  servers, and servers which receive it update the label for that tag. %in the local storage.} 
The three phases of PUT require quorums of  $q_1,q_2,q_3$, resp., responses to complete.  Servers respond to queries from GETs/PUTs only with  latest tag labeled `fin' in their lists. A GET operates in two phases, the first phase to acquire the highest tag labeled `fin' and the second to acquire the chunks for that tag, decode the value and do a write-back. The two phases of GET require responses from quorums of size $q_1,q_4$, resp. In the write-back phase, CAS only sends a `fin' label with the tag, unlike ABD which sends the entire value. %\bu{For Viveck: But $q_4$ servers send back chunks while in ABD servers only send acks. Clarify this additional detail/associated trade-off?} 
\vc{In fact, the structural differences between ABD and CAS protocols translates to lower communication costs for CAS even if $k=1$ (i.e., replication) is used as compared to ABD, with the penalty of incurring higher PUT latency due to the additional phase (\vc{See Table \ref{table:comparison}}). This variation between ABD and CAS offers LEGOStore further flexibility in adapting to workloads as demonstrated in Section~\ref{sec:opt-ins}.}
Similar to ABD, we also employ an "Optimized GET" for CAS that enables some (potentially many) GET operations to complete in only one phase. This optimized GET is based on a client-side cache (recall a client is different from a user, cf. Section~\ref{sec:arch}) for the value  computed in second phase of GET.  LEGOStore exploits these  differences to reduce costs based on if the workload is read- or write-intensive. On the server-side protocol, unlike ABD where a server simply replaces a value with a higher tagged value, CAS  requires servers to store a history of the codeword symbols corresponding to multiple versions, and then garbage collect (GC) older versions at a later point. %In theory, the storage overhead of GC grows with the number of concurrent operations to that specific key. 
However, in practice, the overhead is negligible for the workloads we study (see Appendix \ref{app:gc} in \cite{legostore-arxiv}, \vc{also remarks in Table \ref{table:comparison}.)}. \vc{The preliminary cost comparison of ABD and CAS in Table \ref{table:comparison} ignores several important aspects of practical key-value stores, in particular the spatial diversity of pricing and latency, flexibility of choosing quorum sizes and locations, and the impact of arrival rates. Our paper refines the insights of Table \ref{table:comparison} in the context of LEGOStore (See Section~\ref{sec:opt} for details).}


==> LegoStore-VLDB22CameraReady-arxiv(3)/3design.tex <==
% \vspace{-5pt}
\section{LEGOStore System Design}
\label{sec:arch}

%\bu{TO DISCUSS: shall we conduct the whole discussion in terms of groups instead of keys?}


\subsection{Interface and Components}
\label{sec:interface}

\begin{comment}
\begin{figure}[!t]
    % \centering
    \includegraphics[width=\linewidth]{figures/Legos.pdf}
    \caption{\bu{NEEDS SEVERAL CHANGES.} An overview of LEGOStore.}
    \label{fig:overview}
\end{figure}
\end{comment}

%\bu{
LEGOStore is a linearizable key-value store spanning a set $\mathcal{D}$ of $D$ DCs of a public cloud provider.%\footnote{The $D$ DCs could even be from multiple cloud providers with minor enhancements to our formulations and prototype implementation. } %Figure~\ref{fig:overview} shows its interface to users and its key internal components. 
Applications using LEGOStore ("users")  link the LEGOStore library that offers them an API comprising the following linearizable operations:

%\begin{itemize}
\squishlist
    \item CREATE(k,v): creates the key {\tt k} using default configuration {\tt c} (we will  define a configuration momentarily) if it doesn't already exist and stores {\tt (k,c)} in the local meta-data server (MDS); returns an error if the key already exists.\footnote{A default configuration uses the nearest DCs for various quorums in terms of their RTTs from the client.}
    \item GET(k): returns value for {\tt k} if {\tt k} exists; else  returns an error.
    \item PUT(k,v): sets value of {\tt k} to {\tt v}; returns error if {\tt k} doesn't exist. 
    \item DELETE(k): removes {\tt k};  returns error if {\tt k} doesn't exist.
\squishend
%\end{itemize}

To service these operations, the library issues RPCs to a LEGOStore "client" within a DC in $\mathcal{D}$. A LEGOStore client implements the client-end of LEGOStore's consistency protocols. A user resident within a DC  in $\mathcal{D}$ would be assisted by a client within the same DC. For users outside of $\mathcal{D}$, a natural choice would be a client in the nearest DC. %As we shall see, however, network pricing differences may sometimes make it more cost-effective to choose a client in a DC that is not the nearest (as long as the users latency SLOs allow this). 
The client assisting a user may change over time (e.g., due to user movement) but only across operations. Since the user-client delay is negligible compared to other RTTs involved in request servicing (recall Table~\ref{tab:net+rtt}), we will ignore it in our modeling.  

In order to service a {\tt GET} or a {\tt PUT} request for a key {\tt k}, a client first determines the "configuration" for {\tt k} which consists of the following elements: (i) replication or erasure coding to be used (and, correspondingly,  ABD or CAS); (ii) the DCs that comprise relevant quorums; and (iii) the identities of the LEGOStore "proxies" within each of these DCs. %; and (iv) operational parameters such as timeouts to detect slow/failed quorum members and the order in which to contact additional DCs if needed. 
Having obtained the configuration, a client issues protocol-specific Remote Procedure Calls (RPCs) to proxies in relevant quorums to service the user request. Each DC's proxy serves as the intermediary between the client and the compute/storage servers that (a) implement the server-end of our consistency protocols and (b) store actual data (replicas for ABD, EC chunks for CAS) along with appropriate tags. 

%It is worth noting that when using replication for a key, unlike some related systems~\cite{cops}, LEGOStore does not replicate the key across all DCs but only stores the copies selectively among carefully chosen subsets. %Additionally, when using replication, it does not shard a given key across DCs but stores copies in their entirety within relevant DCs. 
%LEGOStore has the following two components for each key: (i) the {\em optimizer} determines a suitable configuration for the key; see Section~\ref{sec:opt}; and (ii) the {\em reconfiguration controller} safely moves a key from its old configuration to its newly determined configuration; see Section~\ref{sec:reconfig-proto}. Due to the composability property of linearizability and how we model latency, both of these are logically separate across keys. Therefore, LEGOStore does not have a centralized optimizer or reconfiguration controller and,
%in fact, the location of the reconfiguration controller can be chosen carefully %relative to the members of the old and new configuration quorums 
%to help keep reconfiguration time small. 
% (see Sections xxx and yyy).} Shahrooz: I think we should explain here that the controller in LEGOStore has the potential to be distributed, but in our prototype, it is not. In general, this section is not exactly what we did! Should I rewrite it?
%}
%Finally, while EC chunks encoding a key are spread across multiple DCs in a manner reminiscent of sharding, one should note the xxx difference. %See illustrative examples for keys A and B in Figure~\ref{fig:overview} which employ replication with $N=3, f=1, q_1=2, q_2=2$ and EC with xxx, resp. 

==> LegoStore-VLDB22CameraReady-arxiv(3)/4opt.tex <==
% \vspace{-5pt}
\subsection{Finding Cost-Effective Configurations}
\label{sec:opt}
\allowdisplaybreaks{
We develop an optimization %formulation 
that determines cost-effective configurations assuming perfect knowledge of workload and system properties. %In Section~\ref{sec:opt-ins}, we use the optimizer to develop an in-depth understanding of the relationship between (i)  choice of replication vs. EC and  associated parameters such as degree of replication, EC parameters, quorum sizes; and (ii) various workload features and system properties. The optimizer is used by mechanisms in Section~\ref{sec:reconfig-whenwhat} to help adapt LEGOStore's operation to dynamism. Due to space constraints, we describe it in detail in Appendix~\ref{app:optimization}.   
%\bu{These need to be checked and have accompanyign text written as promised in Section 3. Also, the "subject to" field in Section 3 needs to be filled in with the correction connstraing numbers. }
Since our protocols operate at a per-key granularity due to the composability of linearizability~\cite{herlihy90}---notice how the ABD and CAS algorithms in  Appendix~\ref{app:ABD} and~\ref{app:cas} of~\cite{legostore-arxiv} are described for a generic key---we can decompose our datastore-wide optimization into smaller optimization problems, one per key.\footnote{Although we design our optimizer for  individual keys, aggregating keys with similar workload features and considering such a "group" of keys in the optimizer may be useful (perhaps even necessary) for LEGOStore to scale to large number of keys.}% sizes. We leave the identification and evaluation of such groups to future work. } So, in the following, we will outline our formulation for a generic key $g\in G$. 

\noindent {\bf Inputs (See Table \ref{tbl:inputsandvars}):} We assume that \legostore~spans $D$ geo-distributed DCs numbered $1, ..., D$. We assume that the following are available at a per-key granularity: (i) overall request arrival rate;  (ii) geographical distribution of requests (specifically, fractions of the overall arrival rate emerging in/near each DC); (iii) fraction of requests that are GET operations; (iv) average object size  and meta-data\footnote{Meta-data transferred over the network can have non-negligible cost/latency implications and that is what we explicitly capture. On the other hand, the storage of meta-data  contributes relatively negligibly to costs and we do not consider those costs.} size; (v) GET and PUT latency SLOs. %\todo{Check if SLO has been expanded before}. 
We assume that SLOs are in terms of %tail latencies (we use the 
$99^{th}$ percentile latencies. % in our evaluation in Section~\ref{sec:eval}).  
We assume that the availability requirement is expressed via the single parameter $f$> 0; \legostore~must continue servicing requests despite up to $f$ DC failures. The system properties considered in our formulation are: (i) inter-DC latencies and prices for network traffic between %\todo{What is the meaning of protocol-client? }protocol-clients (or just clients) and protocol-servers (or just servers)
clients and servers; (ii) storage; (iii) computational resources in the form of  virtual machines (VMs). %We list these inputs in Table~\ref{tbl:inputsandvars}. 

\begin{table}[!t]
\footnotesize
%\centering
%\resizebox{\textwidth}{!}
\caption{Input and decision variables used by \legostore's optimization. %\bu{CHECK: I have changed $v_i$ into a real. See reasoning offered under "A Detailed Look at our Objective."}
}
% \vspace{-0.1in}
\centering
\begin{tabular}{|p{0.7cm}|p{12cm}|p{1cm}|}
  \hline
 \cellcolor[HTML]{D9D9FF}{\bf \small Input} & \cellcolor[HTML]{D9D9FF}{\bf \small Interpretation} & \cellcolor[HTML]{D9D9FF}{\bf \small Type}\\ 
\hline\hline
$D $ & Number of data centers & integer\\\hline
$\mathcal{D} $ & Set of data centers numbered $1, ..., D$& set\\\hline
$l_{ij}$ & Latency from DC $i$ to DC $j$ (RTT/2) & real\\\hline
$B_{ij}$ & Bandwidth between DC $i$ and DC $j$  %\s{(need to get the numbers to check for asymmetry)}
& real\\\hline
$\mathcal{G}$ & Set of keys & set\\\hline
$\lambda_g$ & Aggregate request arrival rate for key $g\in \mathcal{G}$ & integer\\\hline
$\rho_g$ & Read-write ratio for $g$ & real [0,1]\\\hline
$\alpha_{ig}$ & Fraction of requests originating at/near DC $i$ for key $g$ & real \\\hline
$o_g$ & Average object size, {\em including} protocol-specific metadata exchanged between a client and a server %per-phase protocol-specific meta data exchanged between a client and a server
& integer\\\hline
$o_m$ & Average protocol-specific metadata exchanged between a client and a server for each phase & integer \\\hline
%$n_g$ & Number of objects making up group $g$ & integer\\
%$\beta_g$ & Fraction of concurrent reads that require the write-back phase for ABD 
%\bu{what about for CAS?}\s{CAS reads don't use write-back. first phase is for getting timestamp and second phase for coded values}
%& real\\
$l_{get}$ & GET latency SLO & real\\\hline
$l_{put}$ & PUT latency SLO & real\\\hline
$f$ & Availability requirement (i.e., number of failed DCs  to tolerate) & integer\\\hline
$p_i^s$ & Storage price (per byte per unit time) for DC $i \in \mathcal{D}$ & real \\\hline
$p^n_{ij}$ & Network price per byte from location $i$ to location $j$& real\\\hline
$p^{v}_i$ & VM price at DC $i$ (simplifying assumption: all VMs of a single size) & real\\\hline
$\theta^v$ & This quantity multiplied by the request arrival rate at DC $i$ captures the VM capacity required at $i$ & real\\
   \hline\hline
\cellcolor[HTML]{D9D9FF}{\bf \small Var.} & \cellcolor[HTML]{D9D9FF}{\bf \small Interpretation} & \cellcolor[HTML]{D9D9FF}{\bf \small Type}\\ 
\hline\hline
$e_g$ & Protocol ($0$ for ABD, $1$ for CAS) for key $g$ & boolean\\\hline
$m_g$ & Length of code (replication factor for ABD) & integer\\\hline
$k_g$ & Dimension of code (equals 1 for replication) & integer\\\hline
$q_{i,g}$ & Quorum size for $i^{\text{th}}$ quorum of key $g$ & integer\\\hline
$v_i$ & Capacity of VMs at DC $i$ & real\\\hline
$\mathbf{iq}^k_g$ & Indicator for data placement for $k^{\text{th}}$ quorum of key $g$. $iq_{ijg}^k=1$ iff DC $j$ in $k^{\text{th}}$ quorum of clients in/near DC $i$ & boolean\\ 
\hline
\end{tabular}
\label{tbl:inputsandvars}
% \vspace{-7pt}
\end{table}


\noindent {\bf Decision Variables:} Our decision variables, as described at the bottom of Table~\ref{tbl:inputsandvars}, help capture all aspects of a valid configuration. These include: (i) boolean variable $e_{g}$ whether this key would be served using ABD, and (ii) variables $\mathbf{iq}_g^{k}$ which DCs constitute various quorums that the chosen algorithm (2 and 4 quorums, resp.,  for ABD and  CAS) requires (see variable $iq_{g}^{k}$ in Table \ref{tbl:inputsandvars}). %\todo{What are $2,4$? Are they the number of quorums?}  


%\bu{For Shahrooz: we are not using $v_i$ anywhere. \shans{the optimizer computes the cost of VMs within each datacenter based on the number of requests they are handling. We can use this parameter to reflect that.} Nor are we describing $C_{g,VM}$ anywhere. Can we discuss what the optimizer implements so I can write about these appropriately? \shans{When works for you?}}

\noindent {\bf Optimization:} Our optimization tries to minimize the cost of operating key $g\in {G}$ in the next \emph{epoch} -- a period of relative stability in workload features. Our objective for key $g\in{G}$, which is cost per unit time during the epoch being considered, is expressed as: %Given the assumption of relatively stable workload properties during an epoch,  the total cost over the epoch is simply obtained by multiplying this quantity by the epoch length (which we also assume to be perfectly known at this stage but relax in Section~\ref{sec:dyn}). %\todo{Forward pointer to where we relax this assumption? Seems like a strong assumption}. 
%Our per-key problem  then is:  

%\todo{Shahrooz/BU: equation numbers in the optimization}

% \vspace{1em}
% \vspace{-0.15in}
\begin{equation}
%\boxed{
%\begin{aligned}
\begin{split}
  \text{minimize}~~~\big(C_{g, get} + C_{g, put} + C_{g, Storage} + C_{g, VM}\big)\\
  \text{s.t.}~~~(\ref{eq:put-cost})-(\ref{eq:get-cas-cost})~~~\text{in Appendix~\ref{app:optimization} of~\cite{legostore-arxiv}}.
%\end{aligned}
%}
\end{split}
\label{eq:opt}
\end{equation}

The first two components of the objective with  $put$ and $get$ in their subscripts denote the networking costs per unit time of PUT and GET operations, resp.,  for key $g$ while the last two denote costs per unit time spent towards storage and computation, resp. \vc{The details of the optimization are in Appendix \ref{app:optimization} of \cite{legostore-arxiv}, we reproduce some representative constraints and equations here. 

%\todo{Put a figure about latency that shows the merits of our optimizer}
The networking cost per unit time of PUTs for key $g$ must be represented differently based on whether ABD or CAS is used: $   C_{g,put} = \underbrace{e_g \cdot C_{g,put,CAS}}_{\textrm{n/w cost if CAS chosen}} + \underbrace{(1-e_g) \cdot C_{g,put,ABD}}_{\textrm{n/w cost if ABD chosen}},$ where,
\allowdisplaybreaks{
\begin{equation*}
\begin{split}
C_{g,put,ABD} = (1-\rho_g) \cdot \lambda_g \sum\limits_{i=1}^D \alpha_{ig}\Big(\underbrace{o_m\sum\limits_{j=1}^D {p^n_{ji} \cdot iq^1_{ijg}}}_{\textrm{n/w cost for phase 1}} + \\
        \underbrace{o_g\sum\limits_{k=1}^D {p^n_{ik} \cdot iq^2_{ikg}}}_{\textrm{n/w cost for phase 2}}\Big).
\end{split}
\end{equation*}
\begin{equation}
\begin{split}
 C_{g,put,CAS} = (1-\rho_g) \cdot \lambda_g  \sum\limits_{i=1}^D
 \alpha_{ig}\Big(o_m\Big(\underbrace{\sum\limits_{j=1}^D{p^n_{ji}} \cdot iq^1_{ijg}}_{\textrm{phase 1}} + \\ 
  \underbrace{\sum\limits_{k=1}^D{p^n_{ik} \cdot iq^3_{ikg}}}_{phase 3}\Big) +  \underbrace{\frac{o_g}{k_g}\sum\limits_{m=1}^D{p^n_{im} \cdot iq^2_{img}}}_{phase 2}\Big).
\end{split}
\end{equation}

}
%The terms $C_{g,put,ABD}$ and $C_{g,put,CAS}$ are designed to capture the intensity of network traffic exchanged between clients and the various quorums of servers they need to interact with per the concerned protocol's idiosyncrasies. 

Note the role played by the key boolean decision variable $iq^k_{ijg}$ whose interpretation is: $iq^k_{ijg}$=1 iff data center $j$ is in the $k^{th}$ quorum for clients in/near data center $i$. 
In the above expressions, $(1-\rho_g) \cdot \lambda_g \cdot \alpha_{ig}$ captures the PUT request rate arising at/near data center $i$ and the $o_m$ and $o_g$ multipliers convert this into bytes per unit time. The terms within the braces model the per-byte network transfer prices. The first term represents network transfer prices that apply to the first phase of the ABD PUT protocol whereas the second term does the same for ABD PUT's second phase. The  term $p^n_{ji} \cdot iq^1_{ijg}$ should be understood as follows: since ABD's first phase involves clients in/near data center $i$ sending relatively small-sized {\em write-query} messages to all servers in their quorum (i.e., quorum 1, hence the 1 in the superscript of $iq$) followed by these servers responding with their (tag, value) pairs, the subscript in $p^n_{ji}$ is selected to denote the price of data transfer from $j$ (for the server at data center $j$) to $i$ (for clients located in/near data center $i$).% the multiplication with $iq^1_{ijg}$ achieves the effect of considering these prices only for data centers that are in the client's read quorum.
The network cost per unit time for CAS is similar, with the number of phases being $3$ and the network cost savings offered by CAS reflected in phase $3$, where the value size $o_g$ is divided by the parameter $k_g.$ The networking costs for GET are presented in Appendix \ref{app:optimization} in \cite{legostore-arxiv}.


 The storage cost is modeled as: $C_{g,storage} = p^s \cdot \big(e_g \cdot m_g \cdot \frac{o_g}{k_g} + (1 - e_g) \cdot m_g \cdot o_g \big),$ see \cite{legostore-arxiv} for explanations. Finally, we consider the  VM costs per unit time for key $g$. Our assumptions on modeling VM costs include: ability of procurement of VMs at fine granularity (see, e.g., \cite{small-vm}) and VM autoscaling \cite{burscale, guo-autoscale} to ensure satisfactory provisioning of VM capacity at each DC.  We assume that this suitable VM capacity chosen by such an autoscaling policy is proportional to the total request arrival rate at data center $i$ for key $g$. With these assumptions, the VM cost for key $g$ at data center $i$ is:   
$C_{g,VM} = \theta^v \cdot \sum\limits_{j=1}^D p_j^v \cdot \lambda_g +\sum\limits_{i=1}^D \alpha_{ig} +\sum\limits_{k=1}^4 iq^k_{ijg},$ where $\theta^v$ is an empirically determined multiplier that estimates VM capacity needed to serve the the request rate arriving at data center $j$ for $g$.  
}
%\bu{forward point to Sec. 6 in a couple of places to claim that our modeling choices appear to be reasonable. }

\vc{\noindent {\bf Constraints:} Our optimization needs to capture the 3 types of constraints related to: (i) ensuring linearizability; (ii) meeting availability guarantees corresponding to the parameter $f$; and (iii) meeting latency SLOs.  
The key modeling choices we make are: (i) to use worst-case latency as a "proxy" for tail latency; and (ii) ignore latency contributors within a data center other than data transfer time (e.g., queuing delays, encoding/ decoding time). For PUT operations in CAS, the constraints are $\forall {i, j, k \in \mathcal{D},}$:


%\bu{explain why there is no need to explicitly take a max here. All latencies are required to be $\le$ SLO implying the max would also be.}
\allowdisplaybreaks{
\begin{equation}
\begin{split}
&\underbrace{iq^1_{ijg} \cdot \Big(l_{ij} + l_{ji} + \frac{o_m}{B_{ji}}\Big)}_{\textrm{Latency of first phase of PUT}} + \underbrace{iq^2_{img}\cdot \Big(l_{im} + {\frac{o_g/k_g}{B_{im}} + l_{mi}\Big)}}_{\textrm{Latency of second phase of PUT}} ~~~~+ \\
&\underbrace{iq^3_{ikg}\cdot \Big(l_{ik} + \frac{o_m}{B_{ik}} + l_{ki}\Big)}_{\textrm{Latency of third phase of PUT}} \leq l_{put}.
\end{split}
\end{equation}}
%For PUT operations in ABD, the constraints are, $\forall {i, j, k, m \in \mathcal{D},}$:
%\begin{equation}
%\label{eq:lat-abd-put}
%\begin{split}
%\underbrace{iq^1_{ijg} \cdot %\Big(l_{ij} + l_{ji} + \frac{o_m}{B_{ji}}\Big)}_{\textrm{Latency of first phase of PUT}} + \underbrace{iq^2_{ikg}\cdot \Big(l_{ik} + l_{ki} + {\frac{o_g}{B_{ik}}\Big)}}_{\textrm{Latency of second phase of PUT}}
% \underbrace{iq^3_{ikg}\cdot \Big(l_{ik} + \frac{o_m}{B_{ik}} + l_{ki}\Big)}_{\textrm{Latency of third phase of PUT}}
%\leq l_{put}.
%\end{split}
%\end{equation}
See Appendix \ref{app:optimization} in \cite{legostore-arxiv} for explanations, and for constraints for PUT operations of ABD, and for GETs.  Linearizability and availability targets manifest as constraints on quorum sizes.}

}

==> LegoStore-VLDB22CameraReady-arxiv(3)/5dyn.tex <==
\subsection{How to Reconfigure?}
\label{sec:reconfig-proto}

LEGOStore uses a %simple 
reconfiguration protocol that transitions chosen keys from their old configurations to their new configurations without violating linearizability. \vc{Unlike our approach, consensus-based protocols such as Raft and Viewstamped Replication~\cite{Ousterhout:2013:SDL:2517349.2522716,liskov2012viewstamped}, implement the key-value store as a log of commands applied sequentially to a replicated state machine. These solutions implement reconfiguration by adding it as a special command to this log.} Thus, when a reconfiguration request is issued, the commands that are issued before the reconfiguration request are first applied to the state machine before executing the reconfiguration. To execute the reconfiguration, the leader transfers the state to the new configuration. After the transfer, it resumes handling of client  commands that are serialized after the reconfiguration request, but replicating the state machine in the new configuration. 
While our approach %to key-value store implementation 
does not involve a replicated log\footnote{Rather than a replicated log, we simply have a replicated single read/write variable per key, which is updated on receiving new values.}, it is possible to develop an approach that inherits the essential idea of consensus-based reconfiguration as follows:  (i) On receiving a reconfiguration request, wait for all ongoing operations to complete, and pause all new operations; 
(ii) Perform the reconfiguration by transferring state from the old to the new configurations; (iii) Resume all operations.

%\bu{Viveck: CHECK: to have embed the following functionality within our servers}: 

   

Under the reasonable assumption that reconfigurations {\em of a given key are performed relatively infrequently},\footnote{{More precisely, we assume that reconfigurations to a key are separated in time by periods that are much longer (several minutes to hours or even longer)  than the time it takes to reconfigure (sub-second to a second, see measurements in Section~\ref{sec:reconf-load}).}} our design goal is to ensure that user performance is not degraded in the common case where the configurations remain static. For this, it is crucial that user operations that are not concurrent with reconfigurations  follow the baseline static protocols without requiring additional steps/phases (such as contacting a controller). %, since our goal is to maintain SLOs %efficient performance in the common case. 
%The reconfiguration protocol in \legostore~is executed  on detecting workload changes to an key (see Section~\ref{sec:reconfig-whenwhat} for details) and transitions the key mechanism from an old configuration to a new configuration. 
Our protocol does not assume any special relation between the old and new configurations. It can handle all types transitions, including changing of the replication factor, EC parameters, quorum structure, and the protocol itself. 

%The design goal of the reconfiguration protocol is 
\vc{We wish to keep the number of communication phases as well as the number of operations affected as small as possible. Towards this, \legostore's reconfiguration protocol improves upon steps (i)-(iii) above.} Reconfigurations are conducted by a controller that reads data from the old configuration and transfers it to the new configuration. {On detecting a workload or system change (See Section~\ref{sec:reconfig-whenwhat} for details), the controller immediately performs the reconfiguration without having to wait for all ongoing operations to complete, i.e., without having to perform step (i).} This enables \legostore~to adapt quickly to  workload changes. Furthermore, steps (ii),(iii) are conducted jointly through a single round of messaging. \vc{In particular, \legostore's protocol  integrates with the underlying protocols of CAS and ABD and piggybacks the reconfiguration requests from the controller along with the actions that read or transfer  the data. \legostore's algorithm is provably linearizable (Appendix \ref{app:reconfig} of~\cite{legostore-arxiv}), and therefore, preserves the correctness of the overall data store.} The algorithm blocks certain concurrent operations and then resumes them on completing the reconfiguration.



The reconfiguration protocol is described formally %and its timeline is depicted visually 
in Appendix \ref{app:reconfig} of ~\cite{legostore-arxiv}. %and depicted visually in Figure~\ref{fig:recon_timeline}. 
We assume that reconfigurations are applied sequentially by the reconfiguration controller (or simply controller). %controller. 
The controller sends a \texttt{reconfig\_query} message to all the servers in the old configuration. \vc{The \texttt{reconfig\_query} message serves to both signal a change in configuration, as well as an internal `get' request for the controller to read a consistent value in order to transfer it to the new configuration.}  On receiving this message, the servers pause all the ongoing operations and respond with the latest value if the old configuration is performing ABD, or the highest tag labeled `fin' if it is performing CAS. The controller waits for a quorum to respond from the old configuration. If the old configuration is performing CAS, then the reconfiguration controller sends a \texttt{reconfiguration\_get} message to servers in the old configuration with the highest tag among the messages received from the quorum \vc{(the quorum size is $N-q_2+1$ if the old configuration is performing ABD and $N-\min(q_3,q_4)+1$ if it is performing CAS).} \vc{A server that receives the \texttt{reconfiguration\_get} message with tag $t$ sends a codeword symbol corresponding to that tag, if it is available locally; else it responds with an acknowledgement. The reconfiguration controller then obtains responses from a quorum of $q_4$ messages and decodes the value from the responses.}%If the old configuration is performing ABD, the server simply picks the highest tag $t_{highest}$ and its corresponding value among responses to its $\texttt{reconfig\_query}$ messages. 
 The controller then proceeds to write the $(tag,value)$ pair to the new configuration, performing encoding if the new configuration involves CAS. On completing writing the value to the new configuration, the controller sends a $\texttt{finish\_reconfig}$ message to servers in the old configuration. On receiving these messages, the servers complete all operations with tag less than or equal to $t_{highest}$ and send $\texttt{operation\_fail}$ messages along with information of new configuration to other pending operations that were paused. On receiving $\texttt{operation\_fail}$ messages, the clients restart the operation in the new configuration.



%The idea of the protocol is to effectively halt ongoing operations to the concerned object and simultaneously perform a read on the old configuration via a \texttt{reconfig\_query} message. Having performed a read on the old configuration, the protocol performs a write to the new configuration; once all the servers in the new configuration have received the value, the controller sends a \texttt{begin\_reconfig} message starting the new configuration. The controller also sends a \texttt{finish\_reconfig} message to the old configuration that will finish certain pending operations in this configuration and retire this configuration.  


% \vspace{-5pt}
\subsection{When and What to Reconfigure?}
\label{sec:reconfig-whenwhat}

%In this section, we describe how \legostore~leverages the optimization formulation and the reconfiguration protocol for online operation in the face of dynamism. 
At the heart of our strategy are these questions: (i) is a key configured poorly for its current or upcoming workload? (ii) if yes, should it be stored using a different configuration?
While our discussion focuses on workload dynamism, our ideas also apply to changes in system/infrastructure properties. % such as inter-DC latencies,  cloud pricing, \bu{and set of available nodes}.   

\noindent {\bf Is a Key Configured Sub-Optimally?} Some workload\- changes can be predicted (e.g., cyclical temporal patterns or domain-specific insights from users) while others can only be determined after they have occurred. Generally speaking, a system such as \legostore~would employ a combination of predictive and reactive approaches for detecting workload changes~\cite{wilkespaper,icac05,burscale}. In this paper, we pursue a purely reactive approach. We employ two types of reactive rules that are indicative of a key being configured poorly: 

\noindent $\bullet$ \underline{\em SLO violations: } If SLO violations for a key are observed for more than a threshold duration or during a window containing a  threshold number of requests, \legostore~chooses to  reconfigure it. % since we consider SLO maintenance to be sacrosanct. 
Section~\ref{sec:reconf-load}, \ref{sec:recon-dcfail} show that LEGOStore's reconfiguration occurs within 1 sec; the threshold should be  set sufficiently larger than this to avoid harmful  oscillatory behavior over-optimizing for transient phenomena. %\bu{We use a threshold duration of  minutes in our prototype because XXX. }
If, in addition to SLO violations, some quorum members are suspected of being slow or having failed, these nodes are removed from consideration when determining the next configuration.  

\noindent $\bullet$ \underline{\em Cost sub-optimality:}  Alternatively, a key's configuration might meet the SLO but the estimated running cost might exceed the expected cost. We consider such sub-optimality to have occurred if the observed cost exceeds modeled cost by more than a threshold percentage as assessed over a window of a certain duration.\footnote{ Detailed exploration of the impact of the thresholds on performance is future work.} %In our prototype, we choose these parameters to be XX\% and YY minutes, resp.,  because XXC}. 
Having determined the need for a change, \legostore~ reconfigures the key based on our {\em cost-benefit analysis} described below. 

\noindent {\bf Should Such a Key be Reconfigured?}   For the case of SLO violations, \legostore~will reconfigure as we consider SLO maintenance to be sacrosanct. %and there is no cost-benefit trade-off to consider.  
In the rest of the discussion, we focus on the case of cost sub-optimality. We  assume that such a key's workload features can be predicted for the near term. In the absence of such predictability---and this applies more generally to any similar system---\legostore's options are limited to using a state-of-the-art latency-oriented optimization (see our baselines ABD Nearest and CAS Nearest in Section~\ref{sec:setup}) that is likely to be able to meet the SLO; the impact of such a heuristic on cost is examined in Section~\ref{sec:opt-ins}. 


Assuming predictability, \legostore~computes the new configuration with the updated workload characteristics using the  optimization framework from Section~\ref{sec:opt}. For an illustrative instance of such decision-making, denote this newly computed configuration as $c_{new}$ and the existing configuration as $c_{exist}$. Let us denote by {\tt Cost}$(c)$ the per time unit cost incurred when using configuration $c$. We assume an additional predicted feature $T_{new}$, the minimum duration for which the predicted workload properties will endure before changing. \legostore~ compares the cost involved in reconfiguring with potential cost savings arising due to it.  Reconfiguring a key entails (a) {\em explicit costs} arising from the addtional data transfer; and (b) {\em implicit costs}  resulting from requests that are slowed down or rejected. An evaluation (see Section~\ref{sec:reconf-load} for details) of our reconfiguration protocol suggests that the number of operations experiencing slowdown is small. 
Therefore, we consider only (a). %A practitioner with access to information needed to quantify (b)~\cite{papersreportingrevenuevslosslatency} can readily enhance our cost estimate to  include them. 

%\todo{Remove the following? and replace by above?: We show in Section~\ref{sec:xx} that (b) is negligible? for a variety of reconfiguration scenarios; our reconfiguration protocol is a crucial enabler of these small overheads. A practitioner with access to information needed to quantify (b) can easily enhance our cost estimate to also include such costs (e.g., some industrial papers have reported a relationship between latency degradation and revenue loss). }
    
\legostore's cost-benefit analysis is simple.  A reconfiguration to $c_{new}$ is carried out if the potential (minimum) cost savings $T_{new} \cdot  \big(${\tt Cost}$(c_{exist})-${\tt Cost}$(c_{new})\big)$ significantly outweigh the explicit cost of reconfiguration as captured by {\tt ReCost}$(c_{old},c_{exist})\cdot (1+\alpha)$. {\tt ReCost}$(.,.)$ is the cost of network transfer induced by our reconfiguration and its calculation involves ideas similar to those presented in our optimizer (see  Appendix~\ref{app:optimization} of~\cite{legostore-arxiv}). The $(1+\alpha)$ multiplier ($\alpha>0$) serves to capture how aggressive or conservative \legostore~ wishes to be.  The efficacy of our heuristics depends on the predictability in workload features and the parameter $T_{new}$. %\bu{In our evaluation, we use $T_{new}$ in the range xx-yy because ...; we use $\alpha$ in the range xx-yy because ...} %We empirically evaluate the impact of prediction errors for these features on the quality of \legostore's decision-making in Appendix~\ref{app:predinacc}. 
%Several  concerns orthogonal to our main interest would be crucial to the efficacy of an operational system based on \legostore's ideas. Among these are the use of suitable prediction techniques and suitable tuning of parameters such as $T_{new}$, $\epsilon$, and SLO/cost violation thresholds. 
%\todo{Do we need this last paragraph?}

%\bu{should we explicitly include some error terms into the cost-benefit analysis and forward point to some insights about sensitivity to prediction errors in Section~\ref{sec:pred  inacc}?}




% \noindent {\bf Per-Key Controller Placement:} Note from Algorithms~\ref{algo:recon_cont}, \ref{algo:recon_server_client} that the  time to complete a reconfiguration (call it $T_{re}$) and the time during which GET/PUT operations are blocked are largely dictated by the RTTs between the controller  and the servers farthest from it in 
% the quorums involved in various phases of the reconfiguration protocol.
% Figure~\ref{fig:recon_timeline} highlights this period when both the old and the new configurations use ABD.
% Careful placement of the controller can lower both of these types of delays. \legostore~employs a simple heuristic which locates the controller for a key to be reconfigured on a DC to minimize $T_{re}$ (modeling it as a sum of the relevant RTTs). 

%The optimizer for a key relies on historical data collected from servers and clients for its decision-making described in Section~\ref{sec:reconfig-whenwhat}. A crash of the key's optimizer, therefore, must be protected against. We leave this to future work as it is orthogonal to our main interest in this paper. 
%The reconfiguration controller, on the other hand, is stateless. 


Algorithms~\ref{algo:recon_cont}, \ref{algo:recon_server_client} of \cite{legostore-arxiv} show that the time to complete a reconfiguration (call it $T_{re}$) is largely dictated by the RTTs between the controller and the servers farthest from it in the quorums involved in various phases of the reconfiguration protocol.
Figure~\ref{fig:recon_timeline} of \cite{legostore-arxiv} highlights this period when both the old and the new configurations use ABD. 
%Careful placement of the controller can lower both of these types of delays.

%\legostore~employs a simple heuristic which locates the controller for a key to be reconfigured on a DC to minimize $T_{re}$ (modeling it as a sum of the relevant RTTs). 


==> LegoStore-VLDB22CameraReady-arxiv(3)/6implementation.tex <==
% \vspace{-5pt}
\section{Salient Implementation Aspects}
\label{sec:impl}

%\bu{

%Need to address: what is the meta data overhead per key? Clarify why LEGOStore doesn't need another key-value store  as an SOSP reviewer had thought.  
%}

We implement our  optimizer %(our heuristic approach) 
using Python3.
% in about 1K LOC;  baselines add another 1K LOC.
Since finding the configurations can be done in parallel with each other, we execute up to 48 instances of the optimizer in parallel spanning 8 \emph{e2-standard-4} GCP VMs.\footnote{Our optimizer takes \bu{XXX} msec for each workload on average for $f$=1.}  We implement our LEGOStore prototype in C++11 using about 5.5K LOC. Our prototype uses the {\tt liberasurecode} library's~\cite{liberasurecode}  Reed-Solomon backend for encoding and decoding data in CAS. 
%Figure~\ref{fig:impl} depicts key software components comprising our LEGOStore prototype.
We refer to LEGOStore's users and clients \& servers of our protocols as its {\em data plane}; we call the per-DC metadata servers, the optimizer and reconfiguration controllers its {\em control plane}. \lego's source code is available under the Apache license 2.0 at \href{https://github.com/shahrooz1997/LEGOstore}{github.com/shahrooz1997/LEGOstore}.

\noindent {\bf Data Plane:} A user application (simply user) needs to link the \lego~library %(instead of the key-value store it was using) 
and ensure it uses \lego's API. The library implements logic for the user to interact with the appropriate (ABD or CAS) client. 
LEGOStore maintains a pool of {\em compute nodes} (VMs) (GCP `custom-1-1024' instance types) that run the client and server protocols and store keys using the RocksDB~\cite{rocksdb} database engine.

Each DC maintains a meta-data server (MDS) locally %in its storage layer 
that contains configurations for keys that the clients within it have served and that have not yet been deleted. {\em LEGOStore does not have to have a centralized MDS} with corresponding freedom from concerns related to the failure of such an MDS. When a client does not find a key in the local MDS, it issues queries to other DCs (e.g., in increasing order of RTTs) to learn the key's configuration.

\noindent {\bf Control Plane:}   LEGOStore's control plane comprises the two types of elements for each key described in Section~\ref{sec:interface}: (i) the optimizer and (ii) the reconfiguration controller. Neither of these components is tied to a particular DC location (e.g., See Section~\ref{sec:reconfig-whenwhat} for discussion regarding controller placement). 


==> LegoStore-VLDB22CameraReady-arxiv(3)/7evaluation.tex <==
% \vspace{-0.1in}
\section{Evaluation}
\label{sec:eval}

%We use our optimizer to derive a variety of insights about the efficacy of EC.
We implement a prototype LEGOStore on the Google Compute Engine (GCE) public cloud and make the code for our prototype as well as the optimizer available  under the Apache license 2.0 at \href{https://github.com/shahrooz1997/LEGOstore}{github.com/shahrooz1997/LEGOstore}. Details of our prototype implementation may be found in Appendix~\ref{app:impl} of \cite{legostore-arxiv}. 
We evaluate LEGOStore in terms of its ability to (i)  lower costs compared to the state-of-the-art; and  (ii) meet latency SLOs. We use  Porcupine~\cite{athalye2017porcupine} for verifying linearizability of execution histories of our prototype.

% \vspace{-5pt}
\subsection{Experimental Setup}
\label{sec:setup}

\noindent {\bf Prototype Setup:} We deploy our LEGOStore  prototype across 9 Google Cloud Platform (GCP) DCs with locations, pairwise RTTs, and resource pricing shown in Tables~\ref{tab:dcs} and~\ref{tab:net+rtt}. We locate our users within these data centers as well for the experiments. 
We conduct extensive validation of the efficacy of the latency and cost modeling underlying our optimizer (Appendix~\ref{app:valid} of~\cite{legostore-arxiv}).

\noindent \textbf{Workloads:}  We employ a custom-built workload\footnote{We do not use an existing workload generator such as YCSB~\cite{ycsb} because we wish to explore a wider workload feature space than covered by available tools. } generator which emulates a user application {with an assumption that it sends requests as per a Poisson process.} We explore a large workload space by systematically varying our workload parameters as follows. %\bu{Why don't we use a real trace?}
\squishlist
\item
    3 per-key sizes in KB: (i) 1, (ii) 10, and (iii) 100;
\item 
    3 per-key read ratios for high-read (HR), read-write (RW), and high-write (HW) workloads, resp.: (i) 30:1, (ii) 1:1, and (iii) 1:30; 
\item 
    3 per-key arrival rates in requests/sec: (i) 50, (ii) 200, and (iii) 500; 
\item
    3 sizes for the overall data: (i) 100 GB, (ii) 1 TB, and (iii) 10 TB. %, based on a poll of typical MySQL deployment sizes~\cite{storage-need}.
\item 
    7 different client distributions: (i) Oregon, (ii) Los Angeles, (iii) Tokyo, (iv) Sydney, (v) Los Angeles and Oregon, (vi) Sydney and Singapore, and (vii) Sydney and Tokyo. 
\squishend

This gives us a total of 567 %(3 object sizes * 3 read ratios * 3 arrival rates * 3 storage sizes * 7 client distributions) 
diverse \emph{basic} workloads for a given availability target and latency SLO. Finally, we also vary the availability target ($f$=1 in this section and $f$=2 in Appendix~\ref{app:addnresults} of~\cite{legostore-arxiv}) % \shans{$f=2$ is not in the paper!} 
and latency SLO (in the range 200 ms---1 sec) in our experiments. %\bu{Shahrooz: check if this sentence should stay} \shans{This is correct. It should stay.} 
Additionally, we use the following customized workloads to explore  particular performance related phenomena: (i) a uniform client distribution across all 9 locations; (ii) workloads related to  Figures~\ref{fig:k}-\ref{fig:recon-lat}; we describe these in the text accompanying these figures. Finally, while our exact metadata size varies slightly between ABD and CAS, we round it up to an overestimated  100 B. % in our optimizer. 

%We assume the metadata (\bu{ideally, this would have been precisely defined in Sections 3 and/or 5}) size to be 100B in our optimization; this is a conservative choice in that the actual metadata size in our prototype is smaller (\bu{why can't we just say what our metadata size is and just use that number?}). \shans{We could, but we don't use the current metadata size in the optimizer. Ideally, we should have two different metadata sizes, one for ABD and one for CAS. For ABD, we need metadata size to reflect the size of the data transferred for timestamp, key, etc. For CAS, metadata size should also reflect the metadata for erasure coding, e.g. chunk id, as well. However, we have only one metadata in the optimizer.}

\noindent \textbf{Baselines:} We would like to compare LEGOStore's efficacy to the most important state-of-the-art approaches. To enable such comparison, we construct the following baselines:
%\squishlist 
%\item 
    
\noindent $\bullet$    \textbf{ABD Fixed and CAS Fixed:} These baselines use only ABD or only CAS, respectively. The baseline employs either a fixed degree of replication or a fixed set of CAS parameters.  These  parameter values ($3$ for ABD and $(5,3)$ for CAS) are the ones chosen  most frequently by our optimizer across our large set of experiments described in Section~\ref{sec:opt-ins}. For these fixed parameters, these baselines pick the DCs  with the smallest average network prices for their quorums, where the average for a DC $i$ is calculated over the price of transferring data to all user locations. %network price of one data center is sum of networks price for transferring data to every other data center) divided by the $9$ - number of data centers in our investigation.  \bu{How is this average calculated? \shans{} Which state of the art are these baselines supposed to capture?} \shans{From our discussion, this baselinse was supposed to be a simple baseline where we don't have our heuristic.}
    A comparison with these baselines demonstrates that merely knowing the right parameters does not suffice---one must pick the actual DCs judiciously. 

%\item 
\noindent $\bullet$    \textbf{ABD Nearest and CAS Nearest:} These baselines also use only ABD or only CAS. 
However, they do not a priori fix the degree of replication or the EC parameters. Instead, we pick the optimized value for each parameter and choose quorums that result in the smallest latencies for the GET/PUT operations ignoring cost concerns. They solve a variant of our optimizer where the objective is latency minimization, expressions involving costs are not considered, and all other constraints are the same.  %\bu{are there state of the art approaches these baselines correspond to? Volley?} 
These baselines serve as representatives of existing works (e.g., Volley~\cite{volley} and  \vc{\cite{Sharov:2015:TMY:2824032.2824047}}) that primarily focus on latency reduction. While the baselines are admittedly not as sophisticated as Volley, our results demonstrate that unbridled focus on latency  can lead to high costs.% in the public cloud. 
    
    
%\item 
\noindent $\bullet$    \textbf{ABD Only Optimal and CAS Only Optimal:} These are our most sophisticated baselines meant to represent state-of-the-art approaches. ABD Only Optimal and CAS Only Optimal are representative of works that optimize replication-based systems such as SPANStore~\cite{spanstore} or EC-based systems such as Pando~\cite{pando}.
% \squishend



%\bu{This is a nice insight but it probably fits better somewhere else. Move it once we know what that better place is. } 
It is instructive to note that our baselines are quite powerful. \vc{In fact, our optimizer picks the lower cost feasible solution among ABD Only Optimal and CAS Only Optimal, so we expect at least one of these baselines to be competitive for any given workload. Yet, we will demonstrate that: (i) these baselines \emph{individually} perform poorly for many of our  workloads; and (ii) the choice of which of the two is better for a particular workload is highly non-trivial.} \







\begin{comment}
\begin{table*}
\centering
\caption{This table shows the latencies predicted by the optimizer and the latencies that come from executing the prototype for one hour. We run workload 7 in Table~\ref{tab:workloads} for 10 minutes to get the prototype results.}
\label{tab:latencies}
\begin{tabular}{|l|l||c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|l||}{Latency (ms)} &
  \cellcolor[HTML]{D9D9FF}\textbf{Tokyo} &
  \cellcolor[HTML]{D9D9FF}\textbf{Sydney} &
  \cellcolor[HTML]{D9D9FF}\textbf{Singapore} &
  \cellcolor[HTML]{D9D9FF}\textbf{Frankfurt} &
  \cellcolor[HTML]{D9D9FF}\textbf{London} &
  \cellcolor[HTML]{D9D9FF}\textbf{Virginia} &
  \cellcolor[HTML]{D9D9FF}\textbf{São Paulo} &
  \cellcolor[HTML]{D9D9FF}\textbf{LA} &
  \cellcolor[HTML]{D9D9FF}\textbf{Oregon} \\ \hline \hline
                            & put       & 396 & 463 & 594 & 445 & 413 & 194 & 499 & 161 & 143 \\ \cline{2-11} 
\multirow{-2}{*}{Optimizer}  & get      & 296 & 324 & 428 & 306 & 282 & 136 & 344 & 135 & 117 \\ \hline \hline
                            & put avg  & 396 & 462 & 586 & 445 & 406 & 191 & 493 & 159 & 142 \\ \cline{2-11} 
                            & get avg  & 298 & 325 & 424 & 308 & 278 & 134 & 342 & 134 & 117 \\ \cline{2-11} 
                            & put 99\% & 411 & 467 & 600 & 451 & 413 & 196 & 507 & 162 & 152 \\ \cline{2-11} 
\multirow{-4}{*}{Prototype} & get 99\% & 312 & 330 & 437 & 310 & 282 & 137 & 346 & 136 & 128 \\ \hline \hline
                            & put avg  & 521 & 982 & 662 & 850 & 816 & 615 & 1253 & 416 & 459 \\ \cline{2-11} 
                            & get avg  & 354 & 683 & 512 & 714 & 688 & 557 & 931 & 346 & 377 \\ \cline{2-11} 
                            & put 99\% & 578 & 1003 & 810 & 875 & 845 & 638 & 1276 & 491 & 521 \\ \cline{2-11} 
\multirow{-4}{*}{\begin{tabular}[c]{@{}>{\cellcolor[rgb]{1,1,1}}c@{}} Prototype\\under\\failure\end{tabular}} & get 99\% & 409 & 702 & 647 & 751 & 713 & 582 & 941 & 425 & 441 \\ \hline

\end{tabular}
\end{table*}
\end{comment}



\begin{figure*}[t]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{subfigure}{\columnwidth}
  \centering
  \includegraphics[width=0.95\columnwidth]{figures/cost_f1_1000ms.pdf}
  \caption{Latency SLO=1 sec.}
\end{subfigure}%
\begin{subfigure}{\columnwidth}
  \centering
  \includegraphics[width=0.95\columnwidth]{figures/cost_f1_200ms.pdf}
  \caption{Latency SLO=200 msec.}
\end{subfigure}}
\caption{ Cumulative count of the normalized cost of our baselines (for our 567 basic workloads) with $f=1$ and two extreme latency SLOs.}
\label{fig:normalized-costs}
\end{figure*}



% \vspace{-0.05in}
\subsection{Insights from Our Optimization}
\label{sec:opt-ins}

\begin{figure*}[ht]
    \includegraphics[width=\textwidth]{figures/SLO_latency.pdf}
    % \vspace{-0.2in}
    \caption{Sensitivity of the optimizer's choice to the latency SLO. We consider 2 object sizes (1KB and 10KB), 8 different client distributions, arrival rate=500 req/sec, and $f$=1. We consider 3 different read ratios (HW, RW, HR defined in Section~\ref{sec:setup}). %\bu{Shahrooz: what is the arrival rate here?\shans{500 req/sec} please change "Client distribution" to "User distribution". Please separate this into two graphs. We have decided to keep the one with 1KB size and f=1 as (a) and 10KB and f=1 as (b). The ones with f=2 will be moved into the appendix. Replace "SLO latency (ms)" with "Latency SLO (msec). Draw circles showing areas where there is an ABD to CAS back to ABD transition so the text can refer to these. Don't embed (a) ... (b) ... in the figure but do it here. Also, say (a) Object size=1KB. (b) Object size=10KB.} \shans{I had to embed the (a) and (b) caption because I wanted to have one legend for both figures.}
    }
    \label{fig:slo-latency}
        % \vspace{-5pt}
\end{figure*}

\subsubsection{The Extent and Nature of Cost Savings}
\label{subsec:nature}

%We discuss an instructive %representative 
%subset of our cost savings results. 
In Figure~\ref{fig:normalized-costs}, we express our optimizer's  cost savings over our baselines  via each  baseline's {\em normalized cost} (cost offered by baseline / cost offered by our optimizer); \vc{note that our optimizer has the lowest cost among all the baselines, so this ratio is at least $1$}. We consider  our collection of 567 basic workloads with $f$=1 and (a) a relaxed SLO of 1 sec and (b) a more stringent SLO of 200 msec. \vc{At least one of the baselines - and consequently, our optimizer - meet the SLOs for all the $567$ workloads chosen}.  We begin by contrasting the first-order strengths and weaknesses of ABD and CAS as they are understood in conventional wisdom. For the relatively relaxed latency SLO of 1 sec in Figure~\ref{fig:normalized-costs}(a), we find that ABD Only Optimal (and other ABD-based variants) have more than twice the cost of our optimizer for more than 300 (i.e, more than half) of our workloads. On the other hand, CAS Only Optimal  closely tracks our optimizer's cost.%\footnote{For this relaxed SLO, even CAS Fixed performs close to the optimizer (recall that this fixed $K$ was chosen as the most frequently suggested value by our optimizer for our basic workloads). %\todo{Maybe we should describe that CAS fixed is this much good because we are using the most often used parameters.}
%} 
That is, as widely held, if high latencies are tolerable, EC can save storage and networking costs. Figure~\ref{fig:normalized-costs}(b), with its far more stringent SLO of 200 msec, confirms another aspect of conventional wisdom.  \vc{CAS only optimal is now simply unable to meet the SLO for many workloads (324 out of 567).} This is expected given its 3-phase PUT operations and larger quorums. {(See similar results with $f$=2 in Figure~\ref{fig:normalized-costs2} of~\cite{legostore-arxiv})).} What is  surprising, however, is that when we focus on the subset of 243 workloads for which CAS Only Optimal is feasible, it proves to be the cost-effective choice---nearly all workloads for which CAS Only Optimal is feasible have a normalized cost of 1. So, even for stringent SLOs, EC does hold the potential of saving costs. Unlike in Figure~\ref{fig:normalized-costs}(a), however, CAS Fixed or CAS Nearest are nowhere close to being as effective as CAS Only Optimal. That is, while EC can be cost-effective for these workloads, its %parameters \shans{parameters for Nearest baselines are chosen based on the optimal configuration. We may want to emphasize this.} and 
quorums need to be chosen carefully rather than via  simple greedy heuristics.\footnote{As a further nuance, only 3 workloads out of 243 use CAS with $k$=1.} %\shans{Not all the CAS configurations use EC. A lot of them use $k=1$ which is the same as replication. But, the optimizer picks CAS because it has a smaller get cost. ABD transmits data in both phases while CAS transmit data only in one phase.}
%\todo{Forward 4.2} \bu{Unsure what is meant by "Forward 4.2", please address. }
%These observations suggest that EC has the potential for cost savings beyond only for relaxed latency settings,  but exposing and exploiting that potential requires a careful understanding of how multiple workload features and system properties affect cost and performance. 
Replication tends to be the less preferred choice for more relaxed  SLOs but, again, there are exceptions. 


\subsubsection{Sensitivity to Latency SLO} 
\label{subsec:latency}

We focus on how the cost-efficacy of ABD vs. CAS depends on the latency SLO by examining the entire range of latencies from 50 msec to 1 sec. Furthermore, we separate out this dependence based on read ratio, availability target and object size. Our selected results are shown in % studying this the overall trend - lower latency requiring ABD/replication and higher latency allowing EC to bring cost savings is also depicted in 
Figure~\ref{fig:slo-latency}. %, which portrays the choice of our optimizer for the various workloads that we tested. 
As expected, as one moves towards more relaxed SLOs,  the optimizer's choice tends to shift from ABD to CAS (recall the 3-phase PUTs and larger quorums in CAS). %Using CAS is feasible only when we have a relatively relaxed latency objective because CAS needs 3 round trips to do write operations. Thus, CAS is not feasible with tight SLO latencies.
The complexity that the figures bring out is {\em when} this transition from replication to EC occurs---we see that, depending on workload features, this transition may never occur (e.g., HW in Figure~\ref{fig:slo-latency}(a)) or may occur at a relatively high latency (e.g., at 575 msec for the uniform user  distribution for RW/HR).\footnote{The reader might be intrigued by the portions of Figure~\ref{fig:slo-latency} highlighted using ovals. Here,  our optimizer's choice shifts from ABD to CAS as the latency SLO is relaxed (as expected) but then it shifts back to ABD! We consider this to be a  quirk of the heuristics embedded in our optimizer rather than a fundamental property of the optimal solution. } In particular, more spatially distributed workloads correspond to a tendency to choose replication over EC; for instance, for workloads with uniformly distributed users,  SLOs smaller than 300 msec are infeasible due to a natural lower bound implied by the inter-DC latencies. 
%\bu{Remarks about where CAS=1 fits in vs. ABD and CAS>1.}
%\bu{ Remarks about a few workloads for which there is a switch from ABD to CAS and then back to ABD. Circle these in Figure 4. I understand that this may not be a property of the optimal solution and an artifact of the heuristic embedded in our optimizer but it still seems worth mentioning. }
%We discuss this aspect in Section~\ref{subsec:asymmetry}. 
We find that $f$ also has a complex impact on the optimizer's choice; see results with $f$=2 in Figure~\ref{fig:slo-latencyf2},  Appendix~\ref{app:addnresults} in \cite{legostore-arxiv}. 

% \vspace{-4pt}
\subsubsection{Read- vs. Write-Intensive Workloads}
\label{subsec:asymmetry}

One phenomenon that visibly stands out in Figure~\ref{fig:slo-latency} is how write-intensive workloads for the  relatively small object sizes (HW in Figure~\ref{fig:slo-latency}(a)) prefer ABD  even for the more relaxed SLOs. This preference of ABD over CAS becomes less  pronounced when we increase the object size to 10KB in  Figure~\ref{fig:slo-latency}(b). Finally, we also observe that read-intensive/moderate workloads tend to prefer CAS ($K$=1) over ABD, even when replication is used.  To understand this asymmetry,  note the following:
%\begin{itemize}[leftmargin=*]
%\squishlist
%\item

\noindent $\bullet$ \textbf{Reads:}     
    Whereas both ABD and CAS have a ``write-back'' phase for read operations, ABD's write-back phase carries data, while CAS's only carries metadata, and thereby incurs much lower network cost. Thus, our optimizer tends to prefer CAS for HR workloads.

%\item
\noindent $\bullet$ \textbf{Writes:} 
    For writes,  CAS  involves 3 phases whereas ABD only requires 2. Since each phase incurs an additional overhead in terms of metadata, the metadata costs for write operations are higher for CAS. Therefore, especially for small object sizes (Figure~\ref{fig:slo-latency}(a)) and write-heavy workloads, our optimizer will tend to  prefer  ABD. 
% \squishend
%\end{itemize}

Collectively, the results in Figure~\ref{fig:slo-latency} convey the significant complexity of choosing between ABD and CAS. Within CAS-friendly workloads, there is further substantial complexity in how the parameter $K$ depends on workload features. 


\begin{figure*}[t]
\centering
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=\columnwidth]{figures/cost_k.pdf}
  \caption{}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=\columnwidth]{figures/k_object_size.pdf}
  \caption{}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=\columnwidth]{figures/k_arrival_rate.pdf}
  \caption{}
\end{subfigure}
\caption{For CAS-based solutions, cost is non-monotonic in $K$ and $K_{opt}$ has a complex relation with object size and arrival rate. Latency SLO is 1 sec.} 
\label{fig:k}
% \vspace{-5pt}
\end{figure*}

\subsubsection{Factors Affecting Optimal Code Dimension \texorpdfstring{$K$}{K}} \label{subsubsec:opt-k-dep} 

We illustrate our findings using the representative results in Figure~\ref{fig:k}(a)-(c) based on a workload with the following features for which CAS is the cost-effective choice:  object size=1KB; datastore size=1TB; arrival rate=200 req/sec; read ratio= RW (50\%); user locations are Sydney and Tokyo; latency SLO=1 sec.  %At the outset, the optimizer results in Figure~\ref{fig:k}(a) indicate that cost is non-monotonic in $K$. The results in Figures~\ref{fig:k}(b) and (c), resp., convey that the optimal $K$ ($K_{opt}$ henceforth) (i) increases with object size; but (ii) and decreases with arrival rate. 
To understand the effects in Figure~\ref{fig:k}(a)-(c), we develop a simple analytical model based on the empirical results (details in Appendix~\ref{app:k}, \cite{legostore-arxiv}). Our model relates cost to $K$, object size ($o$), arrival rate ($\lambda$), and $f$ as follows:
\begin{equation}
    cost = \Big(c_1 \cdot \lambda \cdot K + c_2 \cdot o \cdot \lambda  \cdot \frac{f}{K} +c_3 \cdot o \cdot \frac{2f}{K} + \overline{c}_{4}\Big). 
\end{equation}
%\vspace{-3pt}
Here, $c_1,c_2,c_3$  are system-specific constants VM cost, network cost, and storage cost, respectively\footnote{$\overline{c}_{4}$ is a constant and does not affect $K_{opt}$.}. Our model captures and helps understand the {\em non-monotonicity of cost  in $K$} seen in Figure~\ref{fig:k}(a). %---there is a ``sweet spot'' for the choice of $K$ that optimizes the cost.  
This behavior emerges because the following cost components move in opposite directions with growing $K$: network and storage costs decrease due to reduction in object size, while VM costs increase due to increase in quorum sizes. Fundamentally, this implies that even under very relaxed latency constraints, the highest value of $K$ is not necessarily optimal \vc{(contrary to the coarse analysis of Table \ref{table:comparison})}. Our model yields the following optimal value of $K$:
$K_{opt} = \sqrt{\frac{ o\cdot f \cdot (c_2 \cdot \lambda + 2 c_3)}{c_1\cdot \lambda}}.
$
Observe that $K_{opt}$ increases with object size\footnote{A qualification to note is that the phenomenon is connected to our modeling choice of having VM cost independent of the object size $o$. E.g., if the VM cost were chosen as an affine function of $o$, then the dependence of $K_{opt}$ on $o$ would diminish.}, which is in agreement with  Figure~\ref{fig:k}(b). %It is worth noting the parallels with key-value stores within a DC \cite{rashmi2016ec}, wherein the \emph{read latency} was noted to be non-monotonic in $K$ due to the tension between parallelism and straggler effect. We observe a similar behavior, but due to fundamentally different factors that are related to  geo-distribution 
We observe a similar qualitative match  between our model-predicted dependence of $K_{opt}$ on arrival rate and that in Figure~\ref{fig:k}(c). $K_{opt}$ is a decreasing function of the arrival rate {$\lambda$}, and saturates to a constant $K^{*}$ when   {$\lambda \to \infty,$ i.e.,} when the storage cost becomes a negligible component of the overall cost. {Interestingly, even for $\lambda \to \infty$, the system does not revert to replication, i.e., $K^{*}$ is not necessarily $1$.} 


\subsubsection{Does EC Necessarily Have Higher Latency Than Replication?}
\label{subsec:ECvsrep}

Conventional wisdom dictates that EC has lower costs than replication but suffers from higher latency.  %The higher latency expected from EC is due to the fact that EC inevitably requires requests contacting  larger number of DCs  than  with replication. 
We show that perhaps surprisingly, this insight does not always lead to the right choices in the geo-distributed setting. Note that for a linearizable store, requests cannot be local~\cite{attiya1994sequential}, and so even with replication, requests need to contact multiple DCs  and the overall latency corresponds to the response time of the farthest DC. Thus, in a geo-distributed scenario where there are multiple DCs at similar distances as the farthest DC in a replication-based system, EC can offer comparable latency at a lower cost. %, and continue to enjoy the reduced costs.
Our optimizer corroborates this insight. Consider a  workload where requests to a million objects of 1 KB come from users  in Tokyo. The workload is HR (read ratio of 97\%) with an arrival rate of 500 req/sec. To tolerate $f$=1 failure, the lowest GET latency achievable via ABD is 139 msec at a cost of $\$1.057\text{ per hour}$, whereas using CAS achieves a GET latency of 160 msec at a cost of $\$0.704\text{ per hour}$ - a cost saving of $33$\% for a mere 21 msec of latency gap. To tolerate $f$=2 failures for the same workload, the lowest GET latency with ABD is 180 msec at a cost of $\$1.254\text{ per hour}$, whereas CAS offers a GET latency of 190 msec at  a cost of $\$0.773\text{ per hour}$ - 38\% lower cost for a mere 10 msec  latency increase.

% \vspace{-4pt}
\subsubsection{Are Nearest DCs Always the Right Choice?} 
\label{sec:nearest}


Our optimizer reveals that, perhaps surprisingly, the naturally appealing approach of using DCs nearest to user locations~\cite{volley} %the requests 
can lead to wasted costs. We describe one such  finding in Appendix~\ref{app:nearest} of~\cite{legostore-arxiv}. 


\begin{figure}[t]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{subfigure}{.5\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{figures/concurrency_RW.pdf}
  \caption{Read ratio=50\%.}
  \label{fig:slo-latency1}
\end{subfigure}%
\begin{subfigure}{.5\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{figures/concurrency_HW.pdf}
  \caption{Read ratio=3.2\%.}
  \label{fig:slo-latency2}
\end{subfigure}}
\caption{LEGOStore is able to ensure that latency offered to a key is robust even at for highly concurrent accesses. Here we plot the latency experienced by clients at the Tokyo location for arrival rates in [20-100] req/sec. %\bu{Are we going to show model-predicted latencies here per Shahrooz's idea?} %We used workload 7 in Table~\ref{tab:workloads}, and change the arrival rate and read ratio. Lines are showing the trend.
}
\label{fig:concurrency}
% \vspace{-20pt}
\end{figure}





% \vspace{-5pt}
\subsection{Scalable Concurrency Handling}

\label{sec:concurrency}

\begin{comment}
\sz{where is the client located for whom the latency is being reported? what is the degree of replication, what are the quorums?} {\shans{I am not sure if you want to add quorums to the text. The following table was added for your reference.}}

\begin{table}[ht]
\begin{tabular}{ccccc}
 & CAS(5,3) &   &            &        \\
Q1 & California & Oregon   &            &        \\
Q2 & Frankfurt  & Virginia & California & Oregon \\
Q3 & Frankfurt  & Virginia & California & Oregon \\
Q4 & Frankfurt  & Virginia & California & Oregon
\end{tabular}
\label{temp:qurorums}
\end{table}
\end{comment}

A distinguishing feature of LEGOStore is that it is designed to provide reliable tail latency even in the face of highly concurrent access to a key. %f there is high concurrency among operations, even if they are to the same key.  
For consensus-based protocols that apply operations sequentially to a replicated state machines one after another, even in the optimistic case where all operations are issued at a leader that does not fail, the latency is expected to grow linearly with the amount of concurrency. Furthermore, in distributed consensus, due to FLP impossibility \cite{FLP}, concurrent operations may endure several (in theory, unbounded) rounds of communication. %In contrast, we expect LEGOStore to have robust tail latency performance even light of concurrency. 


To validate our expectation of robust tail latency even under high concurrency, we increase the arrival rate for the \emph{same key} with object size 1 KB. The object is configured to use CAS(5, 3) with DCs in Singapore, Frankfurt, Virginia, California, and Oregon. In particular, requests from uniformly-distributed user locations come to the single key. We run the experiments for both HW and RW for a period of 1 minute for each arrival rate. We plot the latency experienced by clients at the Tokyo location against arrival rate in  Figure~\ref{fig:concurrency}. LEGOStore demonstrates a remarkable robustness of the latency of operations. Even for an arrival rate of 100 req/sec to the same key, every operation completes and we see no degradation in performance for the average and tail latencies. We recorded a maximum concurrency of 142 write operations on one key for an arrival rate of 100 req/sec and 30:1 write ratio. Little's law suggests an average concurrency of around 60 operations for this experiment. Note the contrast with consensus-based protocols, where the tail latency is crucially dependent on limited concurrency for a given key. {E.g., in \cite{pando} Figure~13, even with somewhat limited concurrency, the  latency of only ``successful'' writes can grow up to 30s without leader fallback,  and at least doubles with leader fallback.}

The similarity of the latency in Figure~\ref{fig:concurrency}(b) which has a HW workload as compared  with the RW workload in  Figure~\ref{fig:concurrency}(a) indicates that our latencies remain robust even if the workload is write heavy. It is also worth noting that Figure~\ref{fig:concurrency} is a further corroboration of the robustness of our modeling in Section~\ref{sec:opt}. Specifically, our model ignores intra-DC phenomena such as queuing, and the robustness of latency despite a high arrival rate shows the overwhelming  significance of the inter-DC RTTs in determining response times.


\subsection{Reconfiguration to Handle Load Change}
\label{sec:reconf-load}

In this subsection and the next, we explore \lego's ability to  perform fast reconfiguration in line with the expectations set in Section~\ref{sec:reconfig-proto}.~% which plots a run of our LEGOStore for ten minutes with two reconfiguration operations.  
We consider a set of 20 keys with similar workloads, each with an object size of 1 KB and $f$=1 to which RW (i.e., read ratio of 50\%) requests  arrive  from 4  locations with the following distribution: Tokyo (30\%), Sydney (30\%), Singapore (30\%), and Frankfurt (10\%). Each user issues one request every 2 seconds on average. Our latency SLOs are 700 msec and 800 msec for GETs and PUTs, respectively. As seen in  Figure~\ref{fig:recon-lat}, till $t$=200 sec, requests arrive at a total rate of 100 req/sec (i.e., 200 users) from the 4 locations. LEGOStore employs configurations with CAS(5,3) for our keys with DCs in Tokyo, Sydney, Singapore, Virginia, and Oregon. The figure plots the latency experienced by users at Sydney and Frankfurt;  users at Singapore and Tokyo experience similar  SLO adherence.  LEGOStore successfully meets SLOs. In fact, a small number of GET requests (shown using a right-facing arrow) see superior performance as they are "optimized" GETs (recall Section~\ref{sec:back}).  At $t$=200 sec, the collective request arrival rate increases 4-fold to 400 req/sec (i.e., 800 users) while all other workload features remain   unchanged. 
We assume that the %optimizer 
controller located at LA issues a reconfiguration without delay on detecting this workload change. For the new workload, LEGOStore's optimizer recommends a new configuration performing ABD with replication factor of $3$ over DCs in Tokyo, Sydney, and Singapore. Across multiple measurements, we find that reconfiguration concludes in less than 1 sec. The breakdown of overall reconfiguration for a sample instance that takes 717 msec is: (i) reconfig query=68 msec; (ii) reconfig finalize=208 msec; (iii) reconfig write=139 msec; (iv) updating metadata=163; and (v) reconfig finish=139 msec.

We examine user experience during and in the immediate aftermath of reconfiguration. We show the latencies experienced by all the users each at the Sydney and Frankfurt locations to isolate the performance degradation experienced at each user location more clearly.% than would be possible if we were to look at all users collectively. %They were run together. They are separated just to have a better figure. Otherwise, there will be dots all over the figure}. %Notice the higher latencies of the PUTs due to the 3 phases involved in CAS as opposed to 2 phases for GETs. 
 A user request experiences one of two types of degradation which mainly depends on when it arrives in relation to the reconfiguration. {\bf Type (i)} A small number of requests (small due to how quick the reconfiguration is) is blocked at the old configuration servers with the possibility of either getting eventually serviced by these old servers or having to restart in the new configuration (see Section~\ref{sec:reconfig-proto}). These are the requests experiencing latencies in the 750 msec - 1 sec range and highlighted using boxes for the GET requests. {\bf Type (ii)} A second possibility applies to all other requests that do not get blocked at the old configuration servers. These requests incur an additional delay of about 200 msec (users in Sydney) and 250 msec (Frankfurt) to acquire the new configuration from LA and are shown using an ovals for the GET requests. This increase in latency happens because the users do not know that a reconfiguration has occurred and try to do an operation with the old configuration, e.g., see requests at $t \sim$ 200 sec experiencing a slight degradation among GET operations from Sydney users.

\subsection{Reconfiguration to Handle DC Failure}
\label{sec:recon-dcfail}

\begin{figure*}[t]
\centering
{
\begin{subfigure}{0.49\columnwidth} \label{fig:recon-lat1}
  \centering
  \includegraphics[width=\columnwidth]{figures/demonstration_get.pdf}
  \caption{GET operations.}
\end{subfigure}%
\begin{subfigure}{0.49\columnwidth} \label{fig:recon-lat2}
  \centering
  \includegraphics[width=\columnwidth]{figures/demonstration_put.pdf}
  \caption{ PUT operations.}
\end{subfigure}}
% \vspace{-3pt}
\caption{The efficacy and performance impact of two reconfigurations is shown for one of 20 keys with similar workloads. The first reconfiguration occurs in response to a 4-fold increase in request arrival rate at $t$=200 sec. The second reconfiguration occurs at $t$=400 sec in response to the Singapore DC failing at $t$=360 sec. The arrows show the optimized GET operations while the squares and ovals respectively highlight two types of performance degradation associated with reconfiguration: (i) requests blocked in the old configuration, and (ii) first request issued by a user after the reconfiguration which needs to acquire the new configuration from the controller at LA. The different colors for the latency dots represent different users. }
\label{fig:recon-lat}
\end{figure*}

When a DC in one of the quorums fails, LEGOStore will send the request to all other DCs participating in the configuration that are not in the quorum. \vc{This will in general be sub-optimal cost-wise and may also fail to meet the SLO. In Appendix~\ref{app:perf-failure}   Figure~\ref{fig:latency-verif} in \cite{legostore-arxiv}, we show a sample result where a DC failure results in such SLO violation.} To alleviate this, upon detecting a failure,\footnote{LEGOStore can work with any existing approach for failure detection. } LEGOStore invokes its optimizer to determine a new cost-effective configuration that discounts the failed DC and then transitions to this new configuration.
Figure~\ref{fig:recon-lat} depicts a scenario where the Singapore DC, a member of both ABD quorums,  fails at $t$=360 sec. We assume that this failure is detected and remediated via a transition to a new configuration using CAS(4,2) at $t$=400 sec.
Again, we find that the transition occurs within a second and has a small adverse impact on request latency--- most requests whose latency exceeds the SLO are of the unavoidable Type (ii). 

\bu{
\subsection{LEGOStore for a Real-World Workload}
\label{sec:realreconf}

In this subsection, we construct our workload using a publicly available dataset collected from Wikipedia's web server~\cite{wikitrace}. This is a read-mostly workload with a highly skewed popularity distribution.  We extract arrival time and request size information from the dataset and interpret each request as a GET or a PUT based on its type. We sample a set of 1550 distinct objects (each interpreted as a key) from the dataset whose aggregate arrival rate can be accommodated by our prototype. We consider workload features for this set of keys over two 1-hour long periods (call these $T_1$ and $T_2$). Since the workload itself does not reveal a distribution of clients, we assume a uniform distribution of clients among 5 of our DCs (Tokyo, Sydney, Singapore, Frankfurt, London) for $T_1$ and a uniform distribution among all 9 DCs for $T_2$. We use our optimizer to determine cost-effective configurations for each of these keys for both of our 1-hour periods. We choose a latency SLO of 750 msec. 


Our findings demonstrate that \lego~offers cost savings over baselines for the Wikipedia workload. We compare the cost offered by the optimizer against our various baselines for all of the 1550 keys in Figure~\ref{fig:wikicomparison} of \cite{legostore-arxiv}. Even for a fixed duration, the results highlight the importance of the optimizer as a variety of different configurations are chosen for different objects - this includes both replication and CAS and different parameters for CAS. Further, with change in client distribution for a given key, \lego's reconfiguration and optimizer couple to ensure sustained cost effectiveness and improvement over baselines. In Figure~\ref{fig:realreconf},  we highlight an illustrative key's performance in our \lego~ prototype over a 20 minute period with the first 10 minutes from $T_1$ and the second 10 minutes from $T_2$. The arrival rate to this key changes from 16 to 35 req/sec.% across these periods. %Combined with the change in client distribution assumed above,
Our optimizer chooses CAS (m=5, k=1) for $T_1$ and CAS (m=8, k=1) for $T_2$. The latter yields a 20\% cost reduction over the former  and triggers a reconfiguration. Figure~\ref{fig:realreconf} is centered around the reconfiguration LEGOStore carries out for this key at t=10 min. Similar to earlier experiments, our prototype accomplishes the reconfiguration within 1.96 seconds with an increase in response times for a small number of requests during the reconfiguration. 

}

\begin{figure}[t]
\centering
\includegraphics[width=0.7\columnwidth]{figures/Figure_1.pdf}
\caption{The efficacy and performance impact of a reconfiguration (at t=10 min) is shown for a  key that we derive from the Wikipedia dataset.}
\label{fig:realreconf}
\end{figure}

\bu{
% \subsection{Cost Overheads of Our Optimizer}
% \label{opt-cost}
We find that our optimizer, itself executed on public cloud VMs, contributes negligibly to the operational cost of LEGOStore. As an illustrative calculation, for the workload in this section we consider extremely frequent reconfigurations occurring once every 5 minutes for the key with the highest arrival rate of 20.16 req/sec. Each invocation of our optimizer costs about \$0.0001 on average (the average optimizer execution time is 18 sec, see Appendix~\ref{app:impl}). This turns out to be a mere 0.48\% the overall costs for this key.
}


==> LegoStore-VLDB22CameraReady-arxiv(3)/8related_work.tex <==

% \vspace{-5pt} 
\section{Related Work}
\label{sec:related}
% Describe the common approaches near-optimal confs

% Pando

%LEGOStore is closely related to, and builds on the ideas of, several related works. %We discuss the most salient of of them here.

%some papers by Doug Terry?



\noindent {\textbf{EC Based Data Storage:}} %Erasure coding based data storage 
%This area has a rich history. 
Several papers have studied the design of in-memory KV stores ~\cite{rashmi2016ec, shankar2017high, lu2017scalable, zhao2016toward, xiang2016joint, chen2017efficient, wang2017wps, Abebe2018ECStoreBT, duan2018scalable}. A significant body of work focuses on minimizing repair costs and encoding/decoding \cite{ClayCodes,wang2019xorinc, bai2019fast, xie2019az,li2019openec, mitra2016partial, Taranov_ECKV, xia2017revisiting, yiu2017erasure, li2017parix, li2017bcstore, duan2018scalable}.
The cost savings offered by %economic benefits of 
EC have motivated its use particularly in production archival (i.e., write-once/rarely)  systems~\cite{huang2012erasure,FacebookF4}. These papers do not focus on consistency aspects that are relevant to workloads with both reads and writes, nor do they study the geo-distributed setting; therefore, the key factors governing their performance are different from us. %In fact, our paper can be interpreted as an analogue of papers such as \cite{rashmi2016ec}  for the geo-distributed setting. 
Strongly consistent EC-based algorithms and KV stores are developed in \cite{GWGR, Hendricks, Dutta, dobre_powerstore, FAB}; however, none of these works study the geo-distributed setting or the public cloud.




%The geo-distributed setting has been explored in the context of erasure coding, particularly with respect to code design, to address the important concern of reducing the amount of data transfer during repair~\cite{ClayCodes}. This aspect is complementary to our work as we are focused on  reducing cost during normal operation of the key-value store. Integrating efficient failure recovery into our work is an important area of future work.

\noindent{\bf  Strongly Consistent Geo-Distributed Storage:} 
There are several strongly consistent geo-distributed KV stores \cite{Spanner,spanstore,giza,pando,gupta2018fogstore,zhang2013transaction}.
SpanStore~\cite{spanstore} develops an optimization  to minimize costs while satisfying latencies for a strongly consistent geo-distributed store on the public cloud.  While there are several technical differences (e.g., SpanStore uses a blocking protocol via locks), the most important advance made by  \lego~ is its  integration of EC into the picture. Besides tuning EC parameters, \lego~ integrates the constraints of structurally more complex EC-based protocols to enable cost savings. Most closely related to our work are  Giza ~\cite{giza} and Pando~\cite{pando}, which are both strongly consistent EC-based geo-distributed data stores. Both data stores modify consensus protocols (Paxos and Fast Paxos) to utilize EC and minimize latency. The most notable difference between these works and \lego~ is that \lego~ is designed to keep  \emph{tail} latency predictable and robust and keep costs low in the face of dynamism.  Since Giza and Pando are based on consensus, they will tend to have  higher latency under  concurrent writes, e.g., for hot objects with high arrival rates. Furthermore, neither Pando nor Giza have an explicit reconfiguration algorithm. 
%\lego's reconfiguration leverages the GET/PUT protocols and piggybacking of messages to quickly  adapt to changes in workloads and system parameters. 
On the other hand, since Giza and Pando use consensus, they offer more complex primitives such as Read-Modify-Writes and versioned objects. A noteworthy comparison point vs. Giza is that it  does not operate in the public cloud and does not contain an optimization framework for cost minimization. 
%\todo{Say something about insights?}
%Another important related work Gryff~\cite{burke2020gryff} develops a provably linearizable protocol that integrates ABD into Paxos, with the goal of minimizing tail latency for simple GET/PUT operations, and yet simultaneously provide the functionality of a read-modify-write at an inferior tail latency. This is complementary to our work. Integrating EC-based protocols such as CAS into Gryff can lead to translation of our cost savings into read-modify-write data stores; we consider it a direction for future work. 

%\balance

\noindent{\bf Reconfiguration:} There is a growing body of work that develops \emph{non-blocking} algorithms for reconfiguration~\cite{nicolaou2019ares,DYNASTORE}. Algorithms in~\cite{nicolaou2019ares,DYNASTORE} require an additional phase of a client to contact a controller/configuration service in the critical path of \emph{every} operation. In LEGOStore, for the common case of operations that are not concurrent with a reconfiguration, the number of phases (and therefore the latency, costs) are identical to the baseline static protocol. \vc{Our algorithm has a resemblance to an adaptation of \cite{RAMBO} in the tutorial \cite{aguilera2010reconfiguring}. That algorithm works mainly for replication and requires clients to propagate values to the new configuration rather than the controller, which can incur larger costs. Our reconfiguration algorithm utilizes concepts/structures that appear in previous algorithms; our main contribution is to adapt the existing algorithms specifically to ABD and CAS in order to keep the reconfiguration latency/costs low and predictable.  In particular, our algorithm piggybacks read/write requests for the reconfiguration along with messages that are sent to block ongoing operations, and makes careful choices on operations that can be completed in older configurations to provably ensure linearizability.} Several works \cite{Sharov:2015:TMY:2824032.2824047,volley,ardekani2014self} design heuristics to determine when and which objects to reconfigure. Sharov et. al~\cite{Sharov:2015:TMY:2824032.2824047} give a method for optimizing the configuration of quorum-based replication schemes, including the placement of the leaders and replica locations for read and write operations as well as transactions. \vc{The paper shares conceptual similarities with \lego's optimization, but was limited to replication-based schemes and focused solely on minimizing latency for placement, whereas we focus  on erasure-coded schemes and include costs in our placement decisions; on the other hand, our methods do not readily apply to systems that support transactions. A similar comparison applies to the replication-oriented optimizers described in~\cite{zakhary18,abede2020, glasbergen18}. }  Volley~\cite{volley} describes techniques for dynamically migrating data among Microsoft's geo-distributed data centers to keep content closer to users and keeping server loads well-balanced. %A key difference in our work is our cost-oriented objective for public cloud operation whereas Volley's formulation is geared towards a private DC setting.  
% \todo{Bhuvan: please fill.}
 
\noindent {\bf Data Placement and Optimization for Public Cloud:} There is a rich area of data placement and tuning of consistency parameters for replication based geo-distributed stores \cite{terry2013consistency, ardekani2014self, spanstore, replication-placement, shankaranarayanan2014performance, Abebe2018ECStoreBT, su2016systematic, ec-geo-placement}. These works expose the role of diverse workloads and costs in system design,  and our optimization framework is  inspired by this body of work. However, most of these references \cite{terry2013consistency, ardekani2014self,spanstore, replication-placement, shankaranarayanan2014performance} only consider replication.  Reference \cite{Abebe2018ECStoreBT} studied placement and parameter optimization for EC \emph{within} a DC; while some insights are qualitatively similar, our geo-distributed setting along with its diversity makes the salient factors that govern performance different. \vc{From an optimization viewpoint, closest are \cite{ec-geo-placement,su2016systematic} which study EC over geo-distributed public clouds; however, they do not consider consistency and related quorums constraints and costs.}



%\todo{Remove these? Emerging work on performance modeling of consensus protocols, e.g., from SIGMOD19: %https://dl.acm.org/doi/10.1145/3299869.3319893
%separates out two typically intertwined aspects of consensus: discovering whether the last write completed, and determining how to resolve any associated uncertainty . This idea works only when the write ratio is unreasonably low. In that case, our optimizer will pick the configuration such that Q4 is equal to k, and since we have optimized get, we will be able to finish the operation in one phase with the smallest size of quorum. }


%\noindent {\bf Other Related Work:} 



==> LegoStore-VLDB22CameraReady-arxiv(3)/9conclusion.tex <==

% \vspace{-5pt}
\section{Conclusion}
\label{sec:future}

We developed LEGOStore, a linearizable geo-distributed key-value store which procured resources from  a public cloud provider. LEGOStore's goal was to offer tail latency SLOs that were predictable and robust in the face of dynamism. 
We focused on salient aspects of EC's benefits for LEGOStore. % for a cost-aware strongly consistent key-value store. % aiming to expose the salient aspects of the benefits and costs of utilization of EC. 
%It is worth noting that that there are 
Several additional aspects of key-value store design  %that have been outside our scope, that are nonetheless 
%relevant to this broad theme and  %performance and cost, and lead to 
constitute interesting future directions. %We briefly discuss them here.    
For instance, LEGOStore's effectiveness depends on a module that detects workload change and then reconfigures based on the detected changes. %In our implementation, we simulated an idealized version of this module that perfectly detects changes in the workload. The design of such a workload change detection module is orthogonal to our paper, and can be performed based on a number of methods \cite{icac05,wilkespaper}. 
Additionally,
we focused on read/write operations and have not implemented read/modify/write (RMW) operations~\cite{hermes}, which inevitably suffer from less robust tail-latency due to FLP impossibility. The recent paper Gryff \cite{burke2020gryff} designs a provably strongly consistent data store with RMW operations and yet provides the favorable tail-latency properties of  ABD for read and write operations. Gryff is based on replication, and the development of a similar system that uses EC is an interesting area of future research. 


\section*{Acknowledgements}

This work was supported in part by a Google Faculty Award, and the NSF under grants CCF-
1553248 and CNS-1717571. We thank  Raj Pandey for his help in Section~\ref{sec:realreconf}. %, particularly in parsing the wikipedia workload and studying the performance of our optimizer on the same.

\begin{comment}{\noindent \textbf{Throughput and Scalability:} A common stress test for key-value stores is throughput---the average number of transactions per second. %An increase in throughput beyond a certain threshold can result in performance degradation especially for poorly designed data stores. 
We tested our prototype for throughputs of up to 2000 requests per second. LEGOStore's algorithms and design allow for unlimited concurrency, and utilization of the system capacity to its maximum extent. Thus, so long as LEGOStore is operated using a well-provisioned system where the compute and IO resources are scaled  appropriately for incident workload, we expect that LEGOStore can support much higher throughputs. % there is no fundamental bottleneck towards further scaling. % without a degradation in performance. 
This is unlike consensus-based systems where high throughput---which results in increased concurrency---can result in severe latency degradation due to FLP impossibility even if the system is well-provisioned. }





Additionally,
we focused on a read and write operations and have not implemented read/modify/write (RMW) operations~\cite{hermes}. Our data store can be used to implement a RMW operation by performing a read, followed by write; however, it would not be strongly consistent. It is worth contrasting LEGOStore with CassandraDB, whose read and write operations uses protocols similar to ABD. Cassandra offers tuneable consistency, and therefore can be operated as a strongly consistent data store (See a use-case in \cite{ Cassandra_blackrock_youtube}). LEGOStore can be interpreted as a cost-effective EC-based alternative to Cassandra,  when the latter is operated as strongly consistent data store for applications with read/write operations. However, Cassandra implements RMW operations and transactions via Paxos, although incurring performance degradation. Indeed, the recent paper Gryff \cite{burke2020gryff} designs a protocol that offers the best of both worlds of consensus protocols and ABD---it provides a provably strongly consistent data store with RMW operations and yet provides the favorable tail-latency properties of  ABD for read and write operations. Gryff is based on replication, and the development of a similar system that uses EC is an area of future research. 

\end{comment}
%\begin{comment}
%\bu{CANDIDATE FOR REMOVAL?}
%\noindent \textbf{Single Round Read and Write Operations:} 
%Consensus-based protocols that use a stable leader such as Raft, VR and leader-based Paxos can be optimized to offer single round read and write operations for the common case, i.e.,  when the leader does not fail and there is limited concurrency. For a fundamentally similar reason, as we have seen in Section~\ref{sec:back}, both ABD and CAS can offer single rounds for read operations via the optimized GET. However, both these protocols require multiple rounds for PUT operations even in the common case. While the leaderless nature of ABD and CAS allows for more flexibility in the geo-distributed setting, it is possible that the nature of protocol design precludes tighter PUT SLOs for certain workloads.  As LEGOStore allows for reconfiguration, an interesting extension worthy of future systems research is to allow for flexible reconfiguration between leader-based and leaderless protocols to allow it to support a greater range of SLOs.
%\end{comment}

\begin{comment}
% \vspace{-0.1in}
\section{Concluding Remarks}
\label{sec:conclus}

We developed LEGOSTore, a linearizable geo-distributed key-value store which procured resources from public clouds. LEGOStore's goal was to offer tail latency SLOs that were predictable and robust in the face of dynamism. To do so at lower cost compared to the state of the art, LEGOStore's optimizer made judicious use of EC (with savings in networking and storage costs). %To meet its latency-related goals, LEGOStore employed non-blocking leaderless linearizability protocols. 
LEGOStore employed a novel reconfiguration protocol that was able to modify configurations in response to workload and system dynamism quickly. Our extensive evaluation offered several insights related to the use of EC in geo-distributed settings and showed that LEGOStore successfully meets its goals. It offered savings in the \sz{xx-yy\%} range over baselines representing the state of the art while meeting tail latency SLOs. LEGOStore's key reconfiguration time was found to be in the  \sz{xx} ms - 1 sec range, allowing for agile adaptation to dynamic conditions.  
\end{comment}


%The confluence of (a) the need to tolerate data center failures and (b) the necessity of communicating with remote data centers for implementing linearizability in the face of such failures, opens up opportunities for erasure coding to match latency SLOs achievable with replication in a wide range of scenarios. Motivated by this insight, we designed \legostore~that selected the redundancy mechanism, linearizability protocol, protocol-related parameters, and data centers for each object in a way best tailored to its needs and properties. A safe reconfiguration protocol and a practical heuristic cost/benefit analysis allowed it to transform objects for keeping costs under control. Our evaluation (i) offered insights that helped us make suitable modeling decisions, (ii) showed moderate to significant cost savings compared to when the only option is replication, and (iii) manifested the robustness of its underlying protocols where there are many concurrent write operations and violating the SLO latency is not an option.

%\section*{Availability}
%\label{sec:avail}
%\noindent We will open source our LEGOStore prototype, documentation, and all information/data to recreate our experiments as soon as the  anonymity-related policy allows us. 

%\section*{Acknowledgements}
%\label{sec:ack}
%This work was supported in part by the NSF under grants \todo{CNS-xxxxxxx, CNS-xxxxxxx, and CNS-xxxxxxx}.

==> LegoStore-VLDB22CameraReady-arxiv(3)/Tables/datacenters.tex <==
\begin{table*}[t]
\centering
\caption{GCP pricing for the data centers used in our experiments. All numbers are in US dollars.}
\label{tab:datacenters}
\begin{minipage}{\textwidth}
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|} 
\hline
\rowcolor[rgb]{0.851,0.851,1} \textbf{Location} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,1}}c@{}}\textbf{Client}\\\textbf{Distribution}\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,1}}c@{}}\textbf{Object}\\\textbf{size}\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,1}}c@{}}\textbf{Storage}\\\textbf{size}\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,1}}c@{}}\textbf{Arrival}\\\textbf{rate}\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,1}}c@{}}\textbf{Read}\\\textbf{ratio}\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,1}}c@{}}\textbf{SLO}\\\textbf{latency}\end{tabular} \\
\hline
\hline
Network transfer price (USD per GB) & Oregon & 1 KB & 1 TB & 500 req/s & 50\% & 1s \\ 
\hline
EC2 - c5.xlarge (USD per hour) & Oregon & 1 & 1 & 1 & 1 & 1 \\ 
\hline
Storage - SSD gp2 (USD per GB per month) & Oregon & 1 & 1 & 1 & 1 & 1 \\
\hline
\end{tabular}
\end{center}
\bigskip
\centering \footnotesize\emph{Source:} \href{https://cloud.google.com/compute/all-pricing}{All pricing | Compute Engine Documentation | Google Cloud}. Date: May 2020.
\end{minipage}
\end{table*}

==> LegoStore-VLDB22CameraReady-arxiv(3)/algorithms/reconfig.tex <==



\begin{figure}
\centering
    \includegraphics[width=0.6\columnwidth]{figures/recon_protocol.pdf}
    % \vspace{-0.1in}
    \caption{ Reconfiguration protocol timeline. The timeline is depicted assuming both configurations are performing replication-based ABD.}
    \label{fig:recon_timeline}
    % \vspace{-7pt}
\end{figure}


{%\footnotesize
\begin{algorithm}
\SetAlgoLined
\DontPrintSemicolon
% \KwResult{Write here the result }

\textbf{Inputs: } old\_config, new\_config

Send \texttt{reconfig\_query} messages to all servers in \texttt{old\_config}

\eIf(\tcc*[f]{CAS}){old\_config.$e_{g}$ == 1}{

    Await responses from $\max(\texttt{old\_config}.N-\texttt{old\_config}.q_3+1, \texttt{old\_config}.N-\texttt{old\_config}.q_4+1)$ servers
    
    Let $t$ denote the highest logical timestamp received
    
    Send \texttt{reconfig\_get}($t$) message to all servers in \texttt{old\_config}
    
    Wait for \texttt{old\_config}$.q_4$ servers to respond
    
    Decode the corresponding value $v$
    
}(\tcc*[f]{ABD}){
    Await responses from $\texttt{old\_config}.N-q_2+1$ servers
    
    Let $t$ denote the received pair with the highest logical timestamp
    
    Let $v$ be the value of pair $t$
    
    % \eIf(\tcc*[f]{CAS}){\texttt{new\_config}$.e_g==1$}{
    
    %     Send $(t, v, 'fin')$ to all servers in \texttt{new\_config}
        
    %     Wait for $\max(\texttt{new\_config}.q_2,$ $ \texttt{new\_config}.q_3)$ servers to respond
    % }(\tcc*[f]{ABD}){
    %     Send the $(t,v)$ pair to all servers in \texttt{new\_config}
        
    %     Wait for $\texttt{new\_config}.q_2$ servers to respond
    % }
}

\eIf(\tcc*[f]{CAS}){\texttt{new\_config}$.e_g==1$}{
    
        Encode the value $v$ to $chunks$ using Reed-Solomon code
        
        Send \texttt{reconfig\_write}($t, chunk[i], 'fin'$) to $server_i$ for all servers in \texttt{new\_config}
        
        Wait for $\max(\texttt{new\_config}.q_2,$ $ \texttt{new\_config}.q_3)$ servers to respond
    }(\tcc*[f]{ABD}){
        Send \texttt{reconfig\_write}($t,v$) pair to all servers in \texttt{new\_config}
        
        Wait for $\texttt{new\_config}.q_2$ servers to respond
    }

Update global metadata (probably local to the controller) to reflect new configuration;

Send a \texttt{finish\_reconfig}$(t, v$, \texttt{new\_config}$)$ message to all servers in \texttt{old\_config}.
% \sh{This is not the same as implementation}

%where $m=(t,v$,\texttt{new\_config}$)$

%  data; \hfill\COMMENT{//vector<string>}
 
 \caption{Reconfig - Controller}
 \label{algo:recon_cont}
\end{algorithm}
}

{%\footnotesize 
\begin{algorithm}
\SetAlgoLined
% \KwResult{Write here the result }
% \textbf{Inputs: } old\_config, new\_config

% \algblock[On]{On receiving}{end}

% \setcounter{AlgoLine}{0}

\SetKwBlock{Onrecreque}{On receiving a \texttt{reconfig\_query}}{end}
\Onrecreque(\tcc*[f]{from controller}){

    Disable all actions for clients for $\texttt{old\_config}$
    
    \eIf(\tcc*[f]{CAS}){\texttt{new\_config}$.e_g==1$}{
        
        Send the highest tag labeled fin to controller
        
    }(\tcc*[f]{ABD}){
        Send stored $(t,v)$ pair to controller
    }
}

\SetKwBlock{Onrecrefin}{On receiving a \texttt{reconfig\_get}($t$)}{end}
\Onrecrefin(\tcc*[f]{from controller}){
    
    \eIf{the server has a locally stored tuple $(t,chunk,*)$}{
        
        If `*' is `pre', change the label to `fin'
        
        Send $(t,chunk)$ to the controller.
        
    }{
        Store $(t,NULL,'fin')$
        
        Send an ack
    }
}

\SetKwBlock{Onrecfinre}{On receiving a \texttt{finish\_reconfig}($t, v$, {\tt new\_config}$)$}{end}
\Onrecfinre(\tcc*[f]{from controller}){
    
    Send an \texttt{(operation\_fail, new\_config)} message to all \texttt{get\_timestamp} queries.
    
    Unblock other queries and respond as described per protocol to every operation with a tag less than or equal to $t$.
    
    Send an \texttt{(operation\_fail, new\_config)} message to all client operations with tag larger than $t$.
    
    % Delete data related to the old configuration. \sh{should we do it?} %ToDo: make sure if you need to do this or not
}

\SetKwBlock{Onrecchunk}{On receiving a \texttt{reconfig\_write}$(t,v)$ or \texttt{reconfig\_write}$(t,chunk,'fin')$ tuple}{end}
\Onrecchunk(\tcc*[f]{from controller}){
    
    Store the tuple
    
    Send an ack \tcc*[f]{To controller}
}

\SetKwBlock{Onrecopfail}{On receiving \texttt{\texttt{operation\_fail}, \texttt{new\_config})} during an operation}{end}
\Onrecopfail(\tcc*[f]{in client}){
    
    Restart the operation with \texttt{new\_config}.
}
 
\caption{Reconfig - Server and Client}
\label{algo:recon_server_client}
\end{algorithm}
}

==> Tables/datacenters.tex <==
\begin{table*}[t]
\centering
\caption{GCP pricing for the data centers used in our experiments. All numbers are in US dollars.}
\label{tab:datacenters}
\begin{minipage}{\textwidth}
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|} 
\hline
\rowcolor[rgb]{0.851,0.851,1} \textbf{Location} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,1}}c@{}}\textbf{Client}\\\textbf{Distribution}\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,1}}c@{}}\textbf{Object}\\\textbf{size}\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,1}}c@{}}\textbf{Storage}\\\textbf{size}\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,1}}c@{}}\textbf{Arrival}\\\textbf{rate}\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,1}}c@{}}\textbf{Read}\\\textbf{ratio}\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,1}}c@{}}\textbf{SLO}\\\textbf{latency}\end{tabular} \\
\hline
\hline
Network transfer price (USD per GB) & Oregon & 1 KB & 1 TB & 500 req/s & 50\% & 1s \\ 
\hline
EC2 - c5.xlarge (USD per hour) & Oregon & 1 & 1 & 1 & 1 & 1 \\ 
\hline
Storage - SSD gp2 (USD per GB per month) & Oregon & 1 & 1 & 1 & 1 & 1 \\
\hline
\end{tabular}
\end{center}
\bigskip
\centering \footnotesize\emph{Source:} \href{https://cloud.google.com/compute/all-pricing}{All pricing | Compute Engine Documentation | Google Cloud}. Date: May 2020.
\end{minipage}
\end{table*}
